The Dirac point electron in zero-gravity Kerr--Newman spacetime

Dirac's wave equation for a point electron in the topologically nontrivial maximal analytically extended electromagnetic Kerr--Newman spacetime is studied in a zero-gravity limit; here, "zero-gravity" means $G\to 0$, where $G$ is Newton's constant of universal gravitation. The following results are obtained: the formal Dirac Hamiltonian on the static spacelike slices is essentially self-adjoint; the spectrum of the self-adjoint extension is symmetric about zero, featuring a continuum with a gap about zero that, under two smallness conditions, contains a point spectrum. Some of our results extend to a generalization of the zero-$G$ Kerr--Newman spacetime with different electric-monopole-to-magnetic-dipole-moment ratio.

==> KTZ_zGKN_I_null1.tex <==
%Title: C:\Users\shadi\Documents\My Projects\null1.fig
%%Created by: fig2dev.exe Version 3.2 Patchlevel 5d
%%CreationDate: Mon Apr 07 23:40:19 2014
%%User: shadi@SHADI-PC (SHADI-PC)
%
%  Created by WinFIG version 5.01 
%  METADATA <version>1.0</version> 
%
\font\thinlinefont=cmr5
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\mbox{\beginpicture
\setcoordinatesystem units <0.50000cm,0.50000cm>
\unitlength=0.50000cm
\linethickness=1pt
\setplotsymbol ({\makebox(0,0)[l]{\tencirc\symbol{'160}}})
\setshadesymbol ({\thinlinefont .})
\setlinear
%  METADATA <id>1</id> 
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\putrule from  5.080 16.510 to 15.240 16.510
}%
%  METADATA <id>2</id> 
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\putrule from  5.080 11.430 to 15.240 11.430
}%
%  METADATA <id>3</id> 
%
% Fig POLYLINE object
%
\linethickness=1pt
\setplotsymbol ({\makebox(0,0)[l]{\tencirc\symbol{'160}}})
{\color[rgb]{0,0,0}\putrule from  5.080 21.590 to 15.240 21.590
}%
%  METADATA <id>4</id> 
%
% Fig POLYLINE object
%
\linethickness=1pt
\setplotsymbol ({\makebox(0,0)[l]{\tencirc\symbol{'160}}})
{\color[rgb]{0,0,0}\putrule from 15.240 21.590 to 15.240  6.315
\putrule from 15.240  6.350 to  5.045  6.350
\putrule from  5.080  6.350 to  5.080 21.590
}%
%  METADATA <id>5</id> 
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot 13.970 16.192 14.446 15.875 /
%
% arrow head
%
\plot 14.200 15.963 14.446 15.875 14.270 16.069 /
%
}%
%  METADATA <id>6</id> 
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\putrule from  5.080 17.462 to  5.080 16.034
%
% arrow head
%
\plot  5.017 16.288  5.080 16.034  5.143 16.288 /
%
}%
%  METADATA <id>7</id> 
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\putrule from 15.240 12.383 to 15.240 10.795
%
% arrow head
%
\plot 15.176 11.049 15.240 10.795 15.304 11.049 /
%
}%
%  METADATA <id>12</id> 
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
\setdashes < 0.1905cm>
{\color[rgb]{0,0,0}\plot  5.080 12.700  5.084 12.706 /
\plot  5.084 12.706  5.091 12.719 /
\plot  5.091 12.719  5.105 12.742 /
\plot  5.105 12.742  5.124 12.776 /
\plot  5.124 12.776  5.150 12.821 /
\plot  5.150 12.821  5.179 12.874 /
\plot  5.179 12.874  5.213 12.933 /
\plot  5.213 12.933  5.249 12.994 /
\plot  5.249 12.994  5.283 13.056 /
\plot  5.283 13.056  5.317 13.115 /
\plot  5.317 13.115  5.349 13.172 /
\plot  5.349 13.172  5.376 13.227 /
\plot  5.376 13.227  5.404 13.278 /
\plot  5.404 13.278  5.429 13.327 /
\plot  5.429 13.327  5.450 13.373 /
\plot  5.450 13.373  5.472 13.418 /
\plot  5.472 13.418  5.493 13.460 /
\plot  5.493 13.460  5.512 13.504 /
\plot  5.512 13.504  5.531 13.547 /
\plot  5.531 13.547  5.546 13.587 /
\plot  5.546 13.587  5.563 13.627 /
\plot  5.563 13.627  5.580 13.669 /
\plot  5.580 13.669  5.594 13.714 /
\plot  5.594 13.714  5.611 13.758 /
\plot  5.611 13.758  5.628 13.807 /
\plot  5.628 13.807  5.645 13.856 /
\plot  5.645 13.856  5.662 13.904 /
\plot  5.662 13.904  5.679 13.957 /
\plot  5.679 13.957  5.698 14.010 /
\plot  5.698 14.010  5.715 14.063 /
\plot  5.715 14.063  5.732 14.118 /
\plot  5.732 14.118  5.751 14.173 /
\plot  5.751 14.173  5.768 14.228 /
\plot  5.768 14.228  5.785 14.283 /
\plot  5.785 14.283  5.802 14.338 /
\plot  5.802 14.338  5.819 14.393 /
\plot  5.819 14.393  5.836 14.446 /
\plot  5.836 14.446  5.850 14.499 /
\plot  5.850 14.499  5.867 14.552 /
\plot  5.867 14.552  5.884 14.605 /
\plot  5.884 14.605  5.901 14.658 /
\plot  5.901 14.658  5.916 14.707 /
\plot  5.916 14.707  5.931 14.755 /
\plot  5.931 14.755  5.948 14.806 /
\plot  5.948 14.806  5.965 14.859 /
\plot  5.965 14.859  5.982 14.912 /
\plot  5.982 14.912  5.999 14.967 /
\plot  5.999 14.967  6.016 15.022 /
\plot  6.016 15.022  6.035 15.077 /
\plot  6.035 15.077  6.054 15.134 /
\plot  6.054 15.134  6.073 15.193 /
\plot  6.073 15.193  6.092 15.251 /
\plot  6.092 15.251  6.113 15.308 /
\plot  6.113 15.308  6.132 15.365 /
\plot  6.132 15.365  6.151 15.422 /
\plot  6.151 15.422  6.170 15.477 /
\plot  6.170 15.477  6.189 15.532 /
\plot  6.189 15.532  6.208 15.585 /
\plot  6.208 15.585  6.225 15.636 /
\plot  6.225 15.636  6.242 15.685 /
\plot  6.242 15.685  6.259 15.731 /
\plot  6.259 15.731  6.276 15.776 /
\plot  6.276 15.776  6.293 15.820 /
\plot  6.293 15.820  6.308 15.862 /
\plot  6.308 15.862  6.325 15.900 /
\plot  6.325 15.900  6.342 15.947 /
\plot  6.342 15.947  6.361 15.994 /
\plot  6.361 15.994  6.378 16.038 /
\plot  6.378 16.038  6.397 16.082 /
\plot  6.397 16.082  6.416 16.125 /
\plot  6.416 16.125  6.435 16.169 /
\plot  6.435 16.169  6.456 16.212 /
\plot  6.456 16.212  6.477 16.256 /
\plot  6.477 16.256  6.500 16.298 /
\plot  6.500 16.298  6.524 16.341 /
\plot  6.524 16.341  6.547 16.381 /
\plot  6.547 16.381  6.572 16.423 /
\plot  6.572 16.423  6.598 16.463 /
\plot  6.598 16.463  6.625 16.502 /
\plot  6.625 16.502  6.651 16.540 /
\plot  6.651 16.540  6.680 16.578 /
\plot  6.680 16.578  6.708 16.614 /
\plot  6.708 16.614  6.737 16.650 /
\plot  6.737 16.650  6.767 16.686 /
\plot  6.767 16.686  6.801 16.722 /
\plot  6.801 16.722  6.828 16.751 /
\plot  6.828 16.751  6.858 16.783 /
\plot  6.858 16.783  6.888 16.815 /
\plot  6.888 16.815  6.919 16.849 /
\plot  6.919 16.849  6.955 16.883 /
\plot  6.955 16.883  6.991 16.919 /
\plot  6.991 16.919  7.027 16.954 /
\plot  7.027 16.954  7.068 16.990 /
\plot  7.068 16.990  7.108 17.029 /
\plot  7.108 17.029  7.148 17.067 /
\plot  7.148 17.067  7.190 17.107 /
\plot  7.190 17.107  7.235 17.145 /
\plot  7.235 17.145  7.277 17.183 /
\plot  7.277 17.183  7.322 17.223 /
\plot  7.322 17.223  7.366 17.261 /
\plot  7.366 17.261  7.408 17.300 /
\plot  7.408 17.300  7.451 17.336 /
\plot  7.451 17.336  7.493 17.371 /
\plot  7.493 17.371  7.533 17.407 /
\plot  7.533 17.407  7.573 17.441 /
\plot  7.573 17.441  7.614 17.475 /
\plot  7.614 17.475  7.652 17.507 /
\plot  7.652 17.507  7.690 17.539 /
\plot  7.690 17.539  7.726 17.568 /
\plot  7.726 17.568  7.766 17.602 /
\plot  7.766 17.602  7.804 17.634 /
\plot  7.804 17.634  7.844 17.666 /
\plot  7.844 17.666  7.885 17.697 /
\plot  7.885 17.697  7.925 17.731 /
\plot  7.925 17.731  7.965 17.763 /
\plot  7.965 17.763  8.007 17.795 /
\plot  8.007 17.795  8.050 17.827 /
\plot  8.050 17.827  8.094 17.856 /
\plot  8.094 17.856  8.139 17.888 /
\plot  8.139 17.888  8.183 17.918 /
\plot  8.183 17.918  8.227 17.945 /
\plot  8.227 17.945  8.274 17.973 /
\plot  8.274 17.973  8.319 17.998 /
\plot  8.319 17.998  8.363 18.023 /
\plot  8.363 18.023  8.410 18.047 /
\plot  8.410 18.047  8.454 18.068 /
\plot  8.454 18.068  8.498 18.087 /
\plot  8.498 18.087  8.543 18.104 /
\plot  8.543 18.104  8.587 18.121 /
\plot  8.587 18.121  8.632 18.136 /
\plot  8.632 18.136  8.678 18.150 /
\plot  8.678 18.150  8.725 18.163 /
\plot  8.725 18.163  8.774 18.174 /
\plot  8.774 18.174  8.824 18.184 /
\plot  8.824 18.184  8.875 18.195 /
\plot  8.875 18.195  8.930 18.203 /
\plot  8.930 18.203  8.985 18.210 /
\plot  8.985 18.210  9.042 18.216 /
\plot  9.042 18.216  9.100 18.222 /
\plot  9.100 18.222  9.159 18.227 /
\plot  9.159 18.227  9.220 18.229 /
\plot  9.220 18.229  9.279 18.231 /
\plot  9.279 18.231  9.339 18.231 /
\plot  9.339 18.231  9.398 18.231 /
\plot  9.398 18.231  9.455 18.229 /
\plot  9.455 18.229  9.512 18.224 /
\plot  9.512 18.224  9.565 18.220 /
\plot  9.565 18.220  9.618 18.216 /
\plot  9.618 18.216  9.667 18.210 /
\plot  9.667 18.210  9.713 18.203 /
\plot  9.713 18.203  9.760 18.195 /
\plot  9.760 18.195  9.802 18.186 /
\plot  9.802 18.186  9.842 18.176 /
\plot  9.842 18.176  9.889 18.163 /
\plot  9.889 18.163  9.936 18.150 /
\plot  9.936 18.150  9.980 18.133 /
\plot  9.980 18.133 10.022 18.117 /
\plot 10.022 18.117 10.065 18.095 /
\plot 10.065 18.095 10.105 18.074 /
\plot 10.105 18.074 10.147 18.051 /
\plot 10.147 18.051 10.185 18.026 /
\plot 10.185 18.026 10.226 18.000 /
\plot 10.226 18.000 10.262 17.973 /
\plot 10.262 17.973 10.300 17.943 /
\plot 10.300 17.943 10.334 17.913 /
\plot 10.334 17.913 10.370 17.884 /
\plot 10.370 17.884 10.401 17.852 /
\plot 10.401 17.852 10.435 17.822 /
\plot 10.435 17.822 10.467 17.791 /
\plot 10.467 17.791 10.499 17.759 /
\plot 10.499 17.759 10.530 17.727 /
\plot 10.530 17.727 10.560 17.697 /
\plot 10.560 17.697 10.590 17.668 /
\plot 10.590 17.668 10.621 17.636 /
\plot 10.621 17.636 10.655 17.602 /
\plot 10.655 17.602 10.689 17.568 /
\plot 10.689 17.568 10.725 17.532 /
\plot 10.725 17.532 10.761 17.496 /
\plot 10.761 17.496 10.799 17.458 /
\plot 10.799 17.458 10.835 17.418 /
\plot 10.835 17.418 10.875 17.380 /
\plot 10.875 17.380 10.914 17.340 /
\plot 10.914 17.340 10.950 17.302 /
\plot 10.950 17.302 10.988 17.261 /
\plot 10.988 17.261 11.024 17.223 /
\plot 11.024 17.223 11.060 17.185 /
\plot 11.060 17.185 11.093 17.149 /
\plot 11.093 17.149 11.127 17.113 /
\plot 11.127 17.113 11.159 17.079 /
\plot 11.159 17.079 11.189 17.046 /
\plot 11.189 17.046 11.218 17.012 /
\plot 11.218 17.012 11.244 16.982 /
\plot 11.244 16.982 11.271 16.952 /
\plot 11.271 16.952 11.297 16.923 /
\plot 11.297 16.923 11.322 16.891 /
\plot 11.322 16.891 11.347 16.859 /
\plot 11.347 16.859 11.373 16.828 /
\plot 11.373 16.828 11.398 16.792 /
\plot 11.398 16.792 11.424 16.756 /
\plot 11.424 16.756 11.449 16.720 /
\plot 11.449 16.720 11.474 16.679 /
\plot 11.474 16.679 11.498 16.639 /
\plot 11.498 16.639 11.523 16.597 /
\plot 11.523 16.597 11.546 16.554 /
\plot 11.546 16.554 11.568 16.510 /
\plot 11.568 16.510 11.591 16.466 /
\plot 11.591 16.466 11.612 16.419 /
\plot 11.612 16.419 11.631 16.370 /
\plot 11.631 16.370 11.650 16.322 /
\plot 11.650 16.322 11.669 16.273 /
\plot 11.669 16.273 11.686 16.220 /
\plot 11.686 16.220 11.705 16.167 /
\plot 11.705 16.167 11.722 16.112 /
\plot 11.722 16.112 11.733 16.072 /
\plot 11.733 16.072 11.745 16.027 /
\plot 11.745 16.027 11.756 15.983 /
\plot 11.756 15.983 11.769 15.934 /
\plot 11.769 15.934 11.779 15.886 /
\plot 11.779 15.886 11.792 15.833 /
\plot 11.792 15.833 11.803 15.778 /
\plot 11.803 15.778 11.813 15.720 /
\plot 11.813 15.720 11.824 15.661 /
\plot 11.824 15.661 11.834 15.598 /
\plot 11.834 15.598 11.843 15.534 /
\plot 11.843 15.534 11.853 15.466 /
\plot 11.853 15.466 11.862 15.399 /
\plot 11.862 15.399 11.870 15.327 /
\plot 11.870 15.327 11.877 15.253 /
\plot 11.877 15.253 11.883 15.179 /
\plot 11.883 15.179 11.889 15.102 /
\plot 11.889 15.102 11.894 15.024 /
\plot 11.894 15.024 11.898 14.946 /
\plot 11.898 14.946 11.902 14.867 /
\plot 11.902 14.867 11.904 14.787 /
\plot 11.904 14.787 11.904 14.707 /
\plot 11.904 14.707 11.906 14.626 /
\plot 11.906 14.626 11.904 14.544 /
\plot 11.904 14.544 11.904 14.463 /
\plot 11.904 14.463 11.900 14.381 /
\plot 11.900 14.381 11.898 14.300 /
\plot 11.898 14.300 11.891 14.218 /
\plot 11.891 14.218 11.887 14.133 /
\plot 11.887 14.133 11.881 14.048 /
\plot 11.881 14.048 11.874 13.983 /
\plot 11.874 13.983 11.866 13.913 /
\plot 11.866 13.913 11.860 13.843 /
\plot 11.860 13.843 11.851 13.773 /
\plot 11.851 13.773 11.843 13.699 /
\plot 11.843 13.699 11.832 13.625 /
\plot 11.832 13.625 11.822 13.551 /
\plot 11.822 13.551 11.811 13.473 /
\plot 11.811 13.473 11.798 13.394 /
\plot 11.798 13.394 11.786 13.314 /
\plot 11.786 13.314 11.771 13.231 /
\plot 11.771 13.231 11.756 13.149 /
\plot 11.756 13.149 11.741 13.064 /
\plot 11.741 13.064 11.724 12.979 /
\plot 11.724 12.979 11.707 12.893 /
\plot 11.707 12.893 11.688 12.806 /
\plot 11.688 12.806 11.671 12.717 /
\plot 11.671 12.717 11.652 12.630 /
\plot 11.652 12.630 11.631 12.541 /
\plot 11.631 12.541 11.612 12.452 /
\plot 11.612 12.452 11.591 12.366 /
\plot 11.591 12.366 11.568 12.277 /
\plot 11.568 12.277 11.546 12.190 /
\plot 11.546 12.190 11.525 12.103 /
\plot 11.525 12.103 11.502 12.018 /
\plot 11.502 12.018 11.479 11.934 /
\plot 11.479 11.934 11.455 11.851 /
\plot 11.455 11.851 11.432 11.769 /
\plot 11.432 11.769 11.409 11.688 /
\plot 11.409 11.688 11.386 11.610 /
\plot 11.386 11.610 11.362 11.532 /
\plot 11.362 11.532 11.337 11.458 /
\plot 11.337 11.458 11.314 11.383 /
\plot 11.314 11.383 11.290 11.309 /
\plot 11.290 11.309 11.265 11.240 /
\plot 11.265 11.240 11.242 11.170 /
\plot 11.242 11.170 11.216 11.100 /
\plot 11.216 11.100 11.193 11.032 /
\plot 11.193 11.032 11.165 10.962 /
\plot 11.165 10.962 11.138 10.892 /
\plot 11.138 10.892 11.110 10.825 /
\plot 11.110 10.825 11.083 10.757 /
\plot 11.083 10.757 11.053 10.689 /
\plot 11.053 10.689 11.024 10.621 /
\plot 11.024 10.621 10.992 10.554 /
\plot 10.992 10.554 10.958 10.488 /
\plot 10.958 10.488 10.924 10.422 /
\plot 10.924 10.422 10.888 10.357 /
\plot 10.888 10.357 10.850 10.291 /
\plot 10.850 10.291 10.812 10.228 /
\plot 10.812 10.228 10.770 10.164 /
\plot 10.770 10.164 10.727 10.103 /
\plot 10.727 10.103 10.683 10.041 /
\plot 10.683 10.041 10.638  9.982 /
\plot 10.638  9.982 10.590  9.925 /
\plot 10.590  9.925 10.541  9.870 /
\plot 10.541  9.870 10.490  9.815 /
\plot 10.490  9.815 10.437  9.764 /
\plot 10.437  9.764 10.382  9.713 /
\plot 10.382  9.713 10.327  9.667 /
\plot 10.327  9.667 10.270  9.620 /
\plot 10.270  9.620 10.211  9.578 /
\plot 10.211  9.578 10.152  9.538 /
\plot 10.152  9.538 10.090  9.500 /
\plot 10.090  9.500 10.027  9.466 /
\plot 10.027  9.466  9.961  9.432 /
\plot  9.961  9.432  9.895  9.402 /
\plot  9.895  9.402  9.830  9.375 /
\plot  9.830  9.375  9.760  9.349 /
\plot  9.760  9.349  9.690  9.326 /
\plot  9.690  9.326  9.618  9.307 /
\plot  9.618  9.307  9.546  9.290 /
\plot  9.546  9.290  9.470  9.273 /
\plot  9.470  9.273  9.394  9.260 /
\plot  9.394  9.260  9.328  9.252 /
\plot  9.328  9.252  9.260  9.243 /
\plot  9.260  9.243  9.191  9.237 /
\plot  9.191  9.237  9.119  9.233 /
\plot  9.119  9.233  9.045  9.231 /
\plot  9.045  9.231  8.966  9.229 /
\plot  8.966  9.229  8.886  9.231 /
\plot  8.886  9.231  8.801  9.233 /
\plot  8.801  9.233  8.712  9.237 /
\plot  8.712  9.237  8.621  9.241 /
\plot  8.621  9.241  8.524  9.250 /
\plot  8.524  9.250  8.422  9.258 /
\plot  8.422  9.258  8.314  9.271 /
\plot  8.314  9.271  8.204  9.284 /
\plot  8.204  9.284  8.086  9.299 /
\plot  8.086  9.299  7.963  9.315 /
\plot  7.963  9.315  7.836  9.332 /
\plot  7.836  9.332  7.703  9.354 /
\plot  7.703  9.354  7.563  9.375 /
\plot  7.563  9.375  7.419  9.398 /
\plot  7.419  9.398  7.271  9.423 /
\plot  7.271  9.423  7.120  9.449 /
\plot  7.120  9.449  6.966  9.476 /
\plot  6.966  9.476  6.807  9.506 /
\plot  6.807  9.506  6.651  9.533 /
\plot  6.651  9.533  6.494  9.563 /
\plot  6.494  9.563  6.337  9.593 /
\plot  6.337  9.593  6.185  9.622 /
\plot  6.185  9.622  6.039  9.650 /
\plot  6.039  9.650  5.897  9.677 /
\plot  5.897  9.677  5.766  9.703 /
\plot  5.766  9.703  5.643  9.728 /
\plot  5.643  9.728  5.533  9.749 /
\plot  5.533  9.749  5.433  9.771 /
\plot  5.433  9.771  5.347  9.787 /
\plot  5.347  9.787  5.275  9.802 /
\plot  5.275  9.802  5.215  9.815 /
\plot  5.215  9.815  5.167  9.823 /
\plot  5.167  9.823  5.133  9.832 /
\plot  5.133  9.832  5.108  9.836 /
\plot  5.108  9.836  5.093  9.840 /
\plot  5.093  9.840  5.084  9.842 /
\plot  5.084  9.842  5.080  9.842 /
}%
%  METADATA <id>13</id> 
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot 15.240 15.240 15.234 15.244 /
\plot 15.234 15.244 15.221 15.255 /
\plot 15.221 15.255 15.196 15.274 /
\plot 15.196 15.274 15.164 15.301 /
\plot 15.164 15.301 15.121 15.335 /
\plot 15.121 15.335 15.073 15.373 /
\plot 15.073 15.373 15.022 15.416 /
\plot 15.022 15.416 14.973 15.456 /
\plot 14.973 15.456 14.925 15.498 /
\plot 14.925 15.498 14.878 15.536 /
\plot 14.878 15.536 14.838 15.574 /
\plot 14.838 15.574 14.800 15.608 /
\plot 14.800 15.608 14.768 15.642 /
\plot 14.768 15.642 14.736 15.674 /
\plot 14.736 15.674 14.709 15.706 /
\plot 14.709 15.706 14.683 15.737 /
\plot 14.683 15.737 14.658 15.769 /
\plot 14.658 15.769 14.635 15.803 /
\plot 14.635 15.803 14.611 15.837 /
\plot 14.611 15.837 14.588 15.873 /
\plot 14.588 15.873 14.565 15.909 /
\plot 14.565 15.909 14.544 15.949 /
\plot 14.544 15.949 14.520 15.989 /
\plot 14.520 15.989 14.499 16.032 /
\plot 14.499 16.032 14.478 16.076 /
\plot 14.478 16.076 14.457 16.121 /
\plot 14.457 16.121 14.438 16.165 /
\plot 14.438 16.165 14.419 16.212 /
\plot 14.419 16.212 14.400 16.256 /
\plot 14.400 16.256 14.383 16.300 /
\plot 14.383 16.300 14.368 16.345 /
\plot 14.368 16.345 14.353 16.387 /
\plot 14.353 16.387 14.340 16.430 /
\plot 14.340 16.430 14.326 16.470 /
\plot 14.326 16.470 14.315 16.510 /
\plot 14.315 16.510 14.302 16.550 /
\plot 14.302 16.550 14.290 16.593 /
\plot 14.290 16.593 14.279 16.633 /
\plot 14.279 16.633 14.268 16.677 /
\plot 14.268 16.677 14.258 16.720 /
\plot 14.258 16.720 14.247 16.766 /
\plot 14.247 16.766 14.237 16.811 /
\plot 14.237 16.811 14.228 16.857 /
\plot 14.228 16.857 14.220 16.904 /
\plot 14.220 16.904 14.211 16.950 /
\plot 14.211 16.950 14.205 16.995 /
\plot 14.205 16.995 14.199 17.039 /
\plot 14.199 17.039 14.192 17.081 /
\plot 14.192 17.081 14.188 17.124 /
\plot 14.188 17.124 14.186 17.164 /
\plot 14.186 17.164 14.184 17.202 /
\plot 14.184 17.202 14.182 17.240 /
\plot 14.182 17.240 14.182 17.276 /
\plot 14.182 17.276 14.182 17.314 /
\plot 14.182 17.314 14.184 17.350 /
\plot 14.184 17.350 14.186 17.386 /
\plot 14.186 17.386 14.190 17.422 /
\plot 14.190 17.422 14.196 17.460 /
\plot 14.196 17.460 14.203 17.496 /
\plot 14.203 17.496 14.211 17.534 /
\plot 14.211 17.534 14.222 17.570 /
\plot 14.222 17.570 14.235 17.606 /
\plot 14.235 17.606 14.247 17.642 /
\plot 14.247 17.642 14.264 17.674 /
\plot 14.264 17.674 14.281 17.708 /
\plot 14.281 17.708 14.300 17.738 /
\plot 14.300 17.738 14.321 17.765 /
\plot 14.321 17.765 14.343 17.793 /
\plot 14.343 17.793 14.368 17.816 /
\plot 14.368 17.816 14.393 17.839 /
\plot 14.393 17.839 14.421 17.858 /
\plot 14.421 17.858 14.446 17.877 /
\plot 14.446 17.877 14.476 17.894 /
\plot 14.476 17.894 14.506 17.909 /
\plot 14.506 17.909 14.541 17.924 /
\plot 14.541 17.924 14.580 17.939 /
\plot 14.580 17.939 14.624 17.954 /
\plot 14.624 17.954 14.673 17.968 /
\plot 14.673 17.968 14.726 17.983 /
\plot 14.726 17.983 14.785 18.000 /
\plot 14.785 18.000 14.848 18.015 /
\plot 14.848 18.015 14.914 18.030 /
\plot 14.914 18.030 14.980 18.045 /
\plot 14.980 18.045 15.045 18.057 /
\plot 15.045 18.057 15.102 18.070 /
\plot 15.102 18.070 15.153 18.081 /
\plot 15.153 18.081 15.191 18.089 /
\plot 15.191 18.089 15.219 18.093 /
\plot 15.219 18.093 15.234 18.095 /
\plot 15.234 18.095 15.240 18.098 /
}%
%  METADATA <id>14</id> 
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
\setsolid
{\color[rgb]{0,0,0}\plot  5.080 12.700  5.082 12.706 /
\plot  5.082 12.706  5.088 12.717 /
\plot  5.088 12.717  5.101 12.740 /
\plot  5.101 12.740  5.118 12.774 /
\plot  5.118 12.774  5.141 12.819 /
\plot  5.141 12.819  5.171 12.876 /
\plot  5.171 12.876  5.207 12.941 /
\plot  5.207 12.941  5.245 13.013 /
\plot  5.245 13.013  5.285 13.089 /
\plot  5.285 13.089  5.328 13.168 /
\plot  5.328 13.168  5.370 13.244 /
\plot  5.370 13.244  5.412 13.320 /
\plot  5.412 13.320  5.453 13.392 /
\plot  5.453 13.392  5.491 13.460 /
\plot  5.491 13.460  5.529 13.523 /
\plot  5.529 13.523  5.565 13.583 /
\plot  5.565 13.583  5.599 13.638 /
\plot  5.599 13.638  5.632 13.691 /
\plot  5.632 13.691  5.664 13.739 /
\plot  5.664 13.739  5.696 13.786 /
\plot  5.696 13.786  5.730 13.830 /
\plot  5.730 13.830  5.762 13.875 /
\plot  5.762 13.875  5.795 13.917 /
\plot  5.795 13.917  5.825 13.955 /
\plot  5.825 13.955  5.857 13.995 /
\plot  5.857 13.995  5.891 14.034 /
\plot  5.891 14.034  5.925 14.074 /
\plot  5.925 14.074  5.961 14.112 /
\plot  5.961 14.112  5.997 14.152 /
\plot  5.997 14.152  6.035 14.192 /
\plot  6.035 14.192  6.073 14.232 /
\plot  6.073 14.232  6.113 14.275 /
\plot  6.113 14.275  6.155 14.315 /
\plot  6.155 14.315  6.198 14.357 /
\plot  6.198 14.357  6.242 14.398 /
\plot  6.242 14.398  6.284 14.440 /
\plot  6.284 14.440  6.329 14.480 /
\plot  6.329 14.480  6.375 14.520 /
\plot  6.375 14.520  6.420 14.561 /
\plot  6.420 14.561  6.464 14.601 /
\plot  6.464 14.601  6.509 14.639 /
\plot  6.509 14.639  6.553 14.677 /
\plot  6.553 14.677  6.598 14.713 /
\plot  6.598 14.713  6.642 14.751 /
\plot  6.642 14.751  6.684 14.785 /
\plot  6.684 14.785  6.727 14.821 /
\plot  6.727 14.821  6.769 14.855 /
\plot  6.769 14.855  6.811 14.889 /
\plot  6.811 14.889  6.854 14.922 /
\plot  6.854 14.922  6.892 14.954 /
\plot  6.892 14.954  6.932 14.986 /
\plot  6.932 14.986  6.972 15.018 /
\plot  6.972 15.018  7.013 15.050 /
\plot  7.013 15.050  7.055 15.081 /
\plot  7.055 15.081  7.097 15.115 /
\plot  7.097 15.115  7.142 15.149 /
\plot  7.142 15.149  7.188 15.183 /
\plot  7.188 15.183  7.235 15.219 /
\plot  7.235 15.219  7.283 15.255 /
\plot  7.283 15.255  7.332 15.291 /
\plot  7.332 15.291  7.383 15.329 /
\plot  7.383 15.329  7.434 15.365 /
\plot  7.434 15.365  7.487 15.403 /
\plot  7.487 15.403  7.540 15.439 /
\plot  7.540 15.439  7.595 15.477 /
\plot  7.595 15.477  7.648 15.515 /
\plot  7.648 15.515  7.703 15.551 /
\plot  7.703 15.551  7.758 15.589 /
\plot  7.758 15.589  7.813 15.625 /
\plot  7.813 15.625  7.868 15.661 /
\plot  7.868 15.661  7.923 15.697 /
\plot  7.923 15.697  7.978 15.731 /
\plot  7.978 15.731  8.033 15.765 /
\plot  8.033 15.765  8.088 15.801 /
\plot  8.088 15.801  8.143 15.835 /
\plot  8.143 15.835  8.198 15.869 /
\plot  8.198 15.869  8.255 15.900 /
\plot  8.255 15.900  8.306 15.932 /
\plot  8.306 15.932  8.357 15.962 /
\plot  8.357 15.962  8.410 15.991 /
\plot  8.410 15.991  8.465 16.021 /
\plot  8.465 16.021  8.520 16.053 /
\plot  8.520 16.053  8.577 16.085 /
\plot  8.577 16.085  8.636 16.116 /
\plot  8.636 16.116  8.697 16.148 /
\plot  8.697 16.148  8.759 16.180 /
\plot  8.759 16.180  8.822 16.212 /
\plot  8.822 16.212  8.888 16.245 /
\plot  8.888 16.245  8.956 16.277 /
\plot  8.956 16.277  9.023 16.309 /
\plot  9.023 16.309  9.091 16.341 /
\plot  9.091 16.341  9.163 16.375 /
\plot  9.163 16.375  9.233 16.404 /
\plot  9.233 16.404  9.305 16.436 /
\plot  9.305 16.436  9.377 16.466 /
\plot  9.377 16.466  9.449 16.495 /
\plot  9.449 16.495  9.521 16.525 /
\plot  9.521 16.525  9.593 16.552 /
\plot  9.593 16.552  9.665 16.578 /
\plot  9.665 16.578  9.735 16.603 /
\plot  9.735 16.603  9.807 16.626 /
\plot  9.807 16.626  9.874 16.650 /
\plot  9.874 16.650  9.944 16.671 /
\plot  9.944 16.671 10.012 16.692 /
\plot 10.012 16.692 10.080 16.711 /
\plot 10.080 16.711 10.147 16.728 /
\plot 10.147 16.728 10.213 16.745 /
\plot 10.213 16.745 10.279 16.760 /
\plot 10.279 16.760 10.346 16.775 /
\plot 10.346 16.775 10.412 16.787 /
\plot 10.412 16.787 10.478 16.800 /
\plot 10.478 16.800 10.545 16.811 /
\plot 10.545 16.811 10.613 16.821 /
\plot 10.613 16.821 10.681 16.830 /
\plot 10.681 16.830 10.751 16.836 /
\plot 10.751 16.836 10.823 16.842 /
\plot 10.823 16.842 10.894 16.849 /
\plot 10.894 16.849 10.966 16.851 /
\plot 10.966 16.851 11.041 16.855 /
\putrule from 11.041 16.855 to 11.115 16.855
\putrule from 11.115 16.855 to 11.191 16.855
\plot 11.191 16.855 11.267 16.853 /
\plot 11.267 16.853 11.343 16.849 /
\plot 11.343 16.849 11.419 16.844 /
\plot 11.419 16.844 11.496 16.838 /
\plot 11.496 16.838 11.570 16.830 /
\plot 11.570 16.830 11.646 16.819 /
\plot 11.646 16.819 11.720 16.808 /
\plot 11.720 16.808 11.794 16.796 /
\plot 11.794 16.796 11.866 16.781 /
\plot 11.866 16.781 11.938 16.766 /
\plot 11.938 16.766 12.008 16.749 /
\plot 12.008 16.749 12.076 16.730 /
\plot 12.076 16.730 12.141 16.711 /
\plot 12.141 16.711 12.207 16.690 /
\plot 12.207 16.690 12.270 16.667 /
\plot 12.270 16.667 12.332 16.643 /
\plot 12.332 16.643 12.393 16.618 /
\plot 12.393 16.618 12.452 16.593 /
\plot 12.452 16.593 12.509 16.565 /
\plot 12.509 16.565 12.569 16.535 /
\plot 12.569 16.535 12.624 16.506 /
\plot 12.624 16.506 12.681 16.474 /
\plot 12.681 16.474 12.736 16.440 /
\plot 12.736 16.440 12.791 16.404 /
\plot 12.791 16.404 12.848 16.366 /
\plot 12.848 16.366 12.903 16.328 /
\plot 12.903 16.328 12.958 16.286 /
\plot 12.958 16.286 13.013 16.241 /
\plot 13.013 16.241 13.070 16.195 /
\plot 13.070 16.195 13.125 16.148 /
\plot 13.125 16.148 13.180 16.097 /
\plot 13.180 16.097 13.236 16.044 /
\plot 13.236 16.044 13.291 15.991 /
\plot 13.291 15.991 13.343 15.936 /
\plot 13.343 15.936 13.396 15.879 /
\plot 13.396 15.879 13.449 15.820 /
\plot 13.449 15.820 13.502 15.761 /
\plot 13.502 15.761 13.551 15.699 /
\plot 13.551 15.699 13.602 15.638 /
\plot 13.602 15.638 13.648 15.574 /
\plot 13.648 15.574 13.695 15.513 /
\plot 13.695 15.513 13.739 15.450 /
\plot 13.739 15.450 13.784 15.386 /
\plot 13.784 15.386 13.824 15.323 /
\plot 13.824 15.323 13.864 15.259 /
\plot 13.864 15.259 13.902 15.196 /
\plot 13.902 15.196 13.940 15.132 /
\plot 13.940 15.132 13.974 15.069 /
\plot 13.974 15.069 14.008 15.007 /
\plot 14.008 15.007 14.042 14.944 /
\plot 14.042 14.944 14.072 14.880 /
\plot 14.072 14.880 14.103 14.817 /
\plot 14.103 14.817 14.129 14.760 /
\plot 14.129 14.760 14.154 14.702 /
\plot 14.154 14.702 14.177 14.643 /
\plot 14.177 14.643 14.203 14.584 /
\plot 14.203 14.584 14.226 14.522 /
\plot 14.226 14.522 14.249 14.461 /
\plot 14.249 14.461 14.273 14.398 /
\plot 14.273 14.398 14.294 14.332 /
\plot 14.294 14.332 14.317 14.264 /
\plot 14.317 14.264 14.338 14.196 /
\plot 14.338 14.196 14.359 14.127 /
\plot 14.359 14.127 14.381 14.055 /
\plot 14.381 14.055 14.402 13.981 /
\plot 14.402 13.981 14.423 13.904 /
\plot 14.423 13.904 14.442 13.826 /
\plot 14.442 13.826 14.461 13.748 /
\plot 14.461 13.748 14.482 13.667 /
\plot 14.482 13.667 14.499 13.587 /
\plot 14.499 13.587 14.518 13.504 /
\plot 14.518 13.504 14.535 13.420 /
\plot 14.535 13.420 14.554 13.335 /
\plot 14.554 13.335 14.571 13.250 /
\plot 14.571 13.250 14.586 13.164 /
\plot 14.586 13.164 14.603 13.079 /
\plot 14.603 13.079 14.618 12.992 /
\plot 14.618 12.992 14.633 12.903 /
\plot 14.633 12.903 14.647 12.816 /
\plot 14.647 12.816 14.662 12.730 /
\plot 14.662 12.730 14.675 12.641 /
\plot 14.675 12.641 14.690 12.552 /
\plot 14.690 12.552 14.702 12.463 /
\plot 14.702 12.463 14.715 12.374 /
\plot 14.715 12.374 14.728 12.285 /
\plot 14.728 12.285 14.738 12.196 /
\plot 14.738 12.196 14.751 12.105 /
\plot 14.751 12.105 14.764 12.012 /
\plot 14.764 12.012 14.774 11.936 /
\plot 14.774 11.936 14.783 11.858 /
\plot 14.783 11.858 14.793 11.779 /
\plot 14.793 11.779 14.804 11.697 /
\plot 14.804 11.697 14.815 11.614 /
\plot 14.815 11.614 14.825 11.529 /
\plot 14.825 11.529 14.834 11.441 /
\plot 14.834 11.441 14.846 11.350 /
\plot 14.846 11.350 14.857 11.256 /
\plot 14.857 11.256 14.867 11.157 /
\plot 14.867 11.157 14.878 11.055 /
\plot 14.878 11.055 14.891 10.950 /
\plot 14.891 10.950 14.903 10.839 /
\plot 14.903 10.839 14.916 10.723 /
\plot 14.916 10.723 14.929 10.605 /
\plot 14.929 10.605 14.942 10.480 /
\plot 14.942 10.480 14.956 10.348 /
\plot 14.956 10.348 14.971 10.215 /
\plot 14.971 10.215 14.986 10.075 /
\plot 14.986 10.075 15.001  9.931 /
\plot 15.001  9.931 15.016  9.783 /
\plot 15.016  9.783 15.033  9.631 /
\plot 15.033  9.631 15.050  9.478 /
\plot 15.050  9.478 15.064  9.322 /
\plot 15.064  9.322 15.081  9.165 /
\plot 15.081  9.165 15.098  9.011 /
\plot 15.098  9.011 15.113  8.856 /
\plot 15.113  8.856 15.128  8.706 /
\plot 15.128  8.706 15.143  8.560 /
\plot 15.143  8.560 15.157  8.422 /
\plot 15.157  8.422 15.172  8.293 /
\plot 15.172  8.293 15.183  8.172 /
\plot 15.183  8.172 15.196  8.064 /
\plot 15.196  8.064 15.204  7.967 /
\plot 15.204  7.967 15.212  7.882 /
\plot 15.212  7.882 15.221  7.811 /
\plot 15.221  7.811 15.227  7.751 /
\plot 15.227  7.751 15.232  7.705 /
\plot 15.232  7.705 15.236  7.671 /
\plot 15.236  7.671 15.238  7.648 /
\putrule from 15.238  7.648 to 15.238  7.631
\plot 15.238  7.631 15.240  7.624 /
\putrule from 15.240  7.624 to 15.240  7.620
}%
%  METADATA <id>15</id> 
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot 15.240 15.240 15.236 15.242 /
\plot 15.236 15.242 15.229 15.248 /
\plot 15.229 15.248 15.215 15.261 /
\plot 15.215 15.261 15.193 15.278 /
\plot 15.193 15.278 15.164 15.304 /
\plot 15.164 15.304 15.124 15.335 /
\plot 15.124 15.335 15.077 15.373 /
\plot 15.077 15.373 15.024 15.418 /
\plot 15.024 15.418 14.963 15.466 /
\plot 14.963 15.466 14.897 15.519 /
\plot 14.897 15.519 14.829 15.574 /
\plot 14.829 15.574 14.760 15.632 /
\plot 14.760 15.632 14.688 15.687 /
\plot 14.688 15.687 14.616 15.744 /
\plot 14.616 15.744 14.546 15.797 /
\plot 14.546 15.797 14.476 15.852 /
\plot 14.476 15.852 14.408 15.903 /
\plot 14.408 15.903 14.343 15.953 /
\plot 14.343 15.953 14.275 16.002 /
\plot 14.275 16.002 14.211 16.049 /
\plot 14.211 16.049 14.146 16.095 /
\plot 14.146 16.095 14.080 16.142 /
\plot 14.080 16.142 14.014 16.188 /
\plot 14.014 16.188 13.947 16.235 /
\plot 13.947 16.235 13.877 16.281 /
\plot 13.877 16.281 13.805 16.328 /
\plot 13.805 16.328 13.733 16.377 /
\plot 13.733 16.377 13.678 16.413 /
\plot 13.678 16.413 13.623 16.449 /
\plot 13.623 16.449 13.568 16.485 /
\plot 13.568 16.485 13.509 16.521 /
\plot 13.509 16.521 13.447 16.559 /
\plot 13.447 16.559 13.386 16.597 /
\plot 13.386 16.597 13.322 16.635 /
\plot 13.322 16.635 13.255 16.673 /
\plot 13.255 16.673 13.187 16.711 /
\plot 13.187 16.711 13.115 16.749 /
\plot 13.115 16.749 13.041 16.789 /
\plot 13.041 16.789 12.967 16.828 /
\plot 12.967 16.828 12.888 16.866 /
\plot 12.888 16.866 12.808 16.904 /
\plot 12.808 16.904 12.725 16.942 /
\plot 12.725 16.942 12.641 16.978 /
\plot 12.641 16.978 12.556 17.014 /
\plot 12.556 17.014 12.467 17.050 /
\plot 12.467 17.050 12.378 17.081 /
\plot 12.378 17.081 12.287 17.115 /
\plot 12.287 17.115 12.194 17.145 /
\plot 12.194 17.145 12.101 17.175 /
\plot 12.101 17.175 12.006 17.200 /
\plot 12.006 17.200 11.910 17.225 /
\plot 11.910 17.225 11.815 17.249 /
\plot 11.815 17.249 11.718 17.268 /
\plot 11.718 17.268 11.621 17.287 /
\plot 11.621 17.287 11.523 17.304 /
\plot 11.523 17.304 11.426 17.316 /
\plot 11.426 17.316 11.328 17.327 /
\plot 11.328 17.327 11.229 17.333 /
\plot 11.229 17.333 11.132 17.340 /
\plot 11.132 17.340 11.034 17.342 /
\putrule from 11.034 17.342 to 10.937 17.342
\plot 10.937 17.342 10.837 17.338 /
\plot 10.837 17.338 10.740 17.331 /
\plot 10.740 17.331 10.643 17.323 /
\plot 10.643 17.323 10.543 17.310 /
\plot 10.543 17.310 10.446 17.295 /
\plot 10.446 17.295 10.346 17.276 /
\plot 10.346 17.276 10.253 17.257 /
\plot 10.253 17.257 10.162 17.236 /
\plot 10.162 17.236 10.069 17.211 /
\plot 10.069 17.211  9.974 17.183 /
\plot  9.974 17.183  9.878 17.156 /
\plot  9.878 17.156  9.781 17.124 /
\plot  9.781 17.124  9.682 17.090 /
\plot  9.682 17.090  9.582 17.054 /
\plot  9.582 17.054  9.481 17.016 /
\plot  9.481 17.016  9.379 16.978 /
\plot  9.379 16.978  9.273 16.938 /
\plot  9.273 16.938  9.169 16.895 /
\plot  9.169 16.895  9.064 16.851 /
\plot  9.064 16.851  8.956 16.806 /
\plot  8.956 16.806  8.850 16.762 /
\plot  8.850 16.762  8.740 16.717 /
\plot  8.740 16.717  8.632 16.671 /
\plot  8.632 16.671  8.524 16.626 /
\plot  8.524 16.626  8.414 16.580 /
\plot  8.414 16.580  8.306 16.535 /
\plot  8.306 16.535  8.198 16.491 /
\plot  8.198 16.491  8.090 16.447 /
\plot  8.090 16.447  7.984 16.404 /
\plot  7.984 16.404  7.878 16.362 /
\plot  7.878 16.362  7.775 16.324 /
\plot  7.775 16.324  7.671 16.286 /
\plot  7.671 16.286  7.569 16.250 /
\plot  7.569 16.250  7.470 16.216 /
\plot  7.470 16.216  7.374 16.184 /
\plot  7.374 16.184  7.279 16.157 /
\plot  7.279 16.157  7.186 16.131 /
\plot  7.186 16.131  7.095 16.108 /
\plot  7.095 16.108  7.008 16.089 /
\plot  7.008 16.089  6.924 16.072 /
\plot  6.924 16.072  6.841 16.059 /
\plot  6.841 16.059  6.761 16.051 /
\plot  6.761 16.051  6.682 16.044 /
\plot  6.682 16.044  6.608 16.042 /
\plot  6.608 16.042  6.538 16.044 /
\plot  6.538 16.044  6.469 16.049 /
\plot  6.469 16.049  6.403 16.059 /
\plot  6.403 16.059  6.337 16.072 /
\plot  6.337 16.072  6.276 16.091 /
\plot  6.276 16.091  6.219 16.112 /
\plot  6.219 16.112  6.164 16.140 /
\plot  6.164 16.140  6.111 16.169 /
\plot  6.111 16.169  6.060 16.205 /
\plot  6.060 16.205  6.013 16.245 /
\plot  6.013 16.245  5.967 16.290 /
\plot  5.967 16.290  5.922 16.341 /
\plot  5.922 16.341  5.880 16.398 /
\plot  5.880 16.398  5.840 16.461 /
\plot  5.840 16.461  5.800 16.529 /
\plot  5.800 16.529  5.762 16.605 /
\plot  5.762 16.605  5.726 16.688 /
\plot  5.726 16.688  5.690 16.777 /
\plot  5.690 16.777  5.656 16.872 /
\plot  5.656 16.872  5.622 16.976 /
\plot  5.622 16.976  5.590 17.086 /
\plot  5.590 17.086  5.558 17.204 /
\plot  5.558 17.204  5.529 17.329 /
\plot  5.529 17.329  5.499 17.462 /
\plot  5.499 17.462  5.469 17.602 /
\plot  5.469 17.602  5.442 17.748 /
\plot  5.442 17.748  5.412 17.903 /
\plot  5.412 17.903  5.387 18.062 /
\plot  5.387 18.062  5.359 18.227 /
\plot  5.359 18.227  5.334 18.396 /
\plot  5.334 18.396  5.309 18.570 /
\plot  5.309 18.570  5.285 18.743 /
\plot  5.285 18.743  5.262 18.919 /
\plot  5.262 18.919  5.241 19.094 /
\plot  5.241 19.094  5.220 19.266 /
\plot  5.220 19.266  5.201 19.435 /
\plot  5.201 19.435  5.182 19.596 /
\plot  5.182 19.596  5.165 19.751 /
\plot  5.165 19.751  5.150 19.895 /
\plot  5.150 19.895  5.137 20.028 /
\plot  5.137 20.028  5.124 20.149 /
\plot  5.124 20.149  5.114 20.256 /
\plot  5.114 20.256  5.105 20.350 /
\plot  5.105 20.350  5.099 20.428 /
\plot  5.099 20.428  5.093 20.494 /
\plot  5.093 20.494  5.088 20.544 /
\plot  5.088 20.544  5.084 20.582 /
\plot  5.084 20.582  5.082 20.608 /
\plot  5.082 20.608  5.080 20.625 /
\putrule from  5.080 20.625 to  5.080 20.633
\putrule from  5.080 20.633 to  5.080 20.637
}%
%  METADATA <id>21</id> 
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  5.175 11.430  7.017  9.525 /
}%
%  METADATA <id>22</id> 
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  5.175 12.668  8.509  9.271 /
}%
%  METADATA <id>23</id> 
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  5.524 13.462  9.716  9.398 /
}%
%  METADATA <id>24</id> 
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  5.874 14.415 10.446  9.874 /
}%
%  METADATA <id>25</id> 
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  6.159 15.367 10.986 10.700 /
}%
%  METADATA <id>26</id> 
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  6.445 16.320 11.335 11.621 /
}%
%  METADATA <id>27</id> 
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  7.017 16.986 11.557 12.573 /
}%
%  METADATA <id>28</id> 
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  7.747 17.526 11.716 13.589 /
}%
%  METADATA <id>29</id> 
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  8.319 18.129 11.811 14.796 /
}%
%  METADATA <id>30</id> 
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  9.493 18.193 11.462 16.510 /
}%
%  METADATA <id>31</id> 
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  5.143 10.192  5.461  9.811 /
}%
%  METADATA <id>32</id> 
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot 14.383 16.224 15.145 15.589 /
}%
%  METADATA <id>33</id> 
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot 14.129 17.558 15.113 16.637 /
}%
%  METADATA <id>34</id> 
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot 14.859 18.034 15.145 17.780 /
}%
%  METADATA <id>16</id> 
%
% Fig TEXT object
%
\put{\SetFigFont{6}{7.2}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\Ga_l$}%
} [lB] at 11.906 13.653
%  METADATA <id>17</id> 
%
% Fig TEXT object
%
\put{\SetFigFont{6}{7.2}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\Ga_r$}%
} [lB] at 13.494 17.462
%  METADATA <id>18</id> 
%
% Fig TEXT object
%
\put{\SetFigFont{6}{7.2}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\cP_l$}%
} [lB] at 14.446 16.669
%  METADATA <id>19</id> 
%
% Fig TEXT object
%
\put{\SetFigFont{6}{7.2}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\cP_r$}%
} [lB] at  6.985 12.859
%  METADATA <id>20</id> 
%
% Fig TEXT object
%
\put{\SetFigFont{6}{7.2}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\cN$}%
} [lB] at 10.160 19.685
%  METADATA <id>35</id> 
%
% Fig TEXT object
%
\put{\SetFigFont{6}{7.2}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\tilde{S}_-$}%
} [lB] at  3.842 12.668
%  METADATA <id>36</id> 
%
% Fig TEXT object
%
\put{\SetFigFont{6}{7.2}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}
$\tilde{S}_+$}%
} [lB] at 15.367 15.208
%  METADATA <id>37</id> 
%
% Fig TEXT object
%
\put{\SetFigFont{6}{7.2}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\tilde{N}_+$}%
} [lB] at 15.367 18.002
%  METADATA <id>38</id> 
%
% Fig TEXT object
%
\put{\SetFigFont{6}{7.2}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\bar{N}_+$}%
} [lB] at 15.399  7.588
%  METADATA <id>39</id> 
%
% Fig TEXT object
%
\put{\SetFigFont{6}{7.2}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\bar{N}_-$}%
} [lB] at  3.873  9.716
%  METADATA <id>40</id> 
%
% Fig TEXT object
%
\put{\SetFigFont{6}{7.2}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\tilde{N}_-$}%
} [lB] at  3.842 20.225
%  METADATA <id>41</id> 
%
% Fig TEXT object
%
\put{\SetFigFont{6}{7.2}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\cN$}%
} [lB] at 12.732 14.732
\linethickness=0pt
\putrectangle corners at  3.810 21.660 and 15.431  6.280
\endpicture}


==> KTZ_zGKN_I_null2.tex <==
%Title: C:\Users\shadi\Documents\My Projects\null2.fig
%%Created by: fig2dev.exe Version 3.2 Patchlevel 5d
%%CreationDate: Mon Apr 07 23:51:03 2014
%%User: shadi@SHADI-PC (SHADI-PC)
%
%  Created by WinFIG version 5.01 
%  METADATA <version>1.0</version> 
%
\font\thinlinefont=cmr5
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\mbox{\beginpicture
\setcoordinatesystem units <0.50000cm,0.50000cm>
\unitlength=0.50000cm
\linethickness=1pt
\setplotsymbol ({\makebox(0,0)[l]{\tencirc\symbol{'160}}})
\setshadesymbol ({\thinlinefont .})
\setlinear
%  METADATA <id>1</id> 
%
% Fig POLYLINE object
%
\linethickness=1pt
\setplotsymbol ({\makebox(0,0)[l]{\tencirc\symbol{'160}}})
{\color[rgb]{0,0,0}\putrule from  5.080 21.590 to 15.240 21.590
}%
%  METADATA <id>2</id> 
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\putrule from  5.080 16.510 to 15.240 16.510
}%
%  METADATA <id>3</id> 
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\putrule from  5.080 11.430 to 15.240 11.430
}%
%  METADATA <id>4</id> 
%
% Fig POLYLINE object
%
\linethickness=1pt
\setplotsymbol ({\makebox(0,0)[l]{\tencirc\symbol{'160}}})
{\color[rgb]{0,0,0}\putrule from 15.240 21.590 to 15.240  6.315
\putrule from 15.240  6.350 to  5.045  6.350
\putrule from  5.080  6.350 to  5.080 21.590
}%
%  METADATA <id>5</id> 
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
\setdashes < 0.1905cm>
{\color[rgb]{0,0,0}\plot 15.240 15.240 15.236 15.240 /
\plot 15.236 15.240 15.223 15.238 /
\plot 15.223 15.238 15.202 15.234 /
\plot 15.202 15.234 15.170 15.229 /
\plot 15.170 15.229 15.124 15.223 /
\plot 15.124 15.223 15.064 15.215 /
\plot 15.064 15.215 14.994 15.204 /
\plot 14.994 15.204 14.910 15.193 /
\plot 14.910 15.193 14.817 15.179 /
\plot 14.817 15.179 14.717 15.164 /
\plot 14.717 15.164 14.611 15.149 /
\plot 14.611 15.149 14.503 15.134 /
\plot 14.503 15.134 14.393 15.117 /
\plot 14.393 15.117 14.285 15.102 /
\plot 14.285 15.102 14.180 15.085 /
\plot 14.180 15.085 14.076 15.071 /
\plot 14.076 15.071 13.978 15.056 /
\plot 13.978 15.056 13.885 15.043 /
\plot 13.885 15.043 13.796 15.030 /
\plot 13.796 15.030 13.712 15.018 /
\plot 13.712 15.018 13.631 15.005 /
\plot 13.631 15.005 13.555 14.994 /
\plot 13.555 14.994 13.483 14.982 /
\plot 13.483 14.982 13.413 14.971 /
\plot 13.413 14.971 13.348 14.963 /
\plot 13.348 14.963 13.282 14.952 /
\plot 13.282 14.952 13.219 14.942 /
\plot 13.219 14.942 13.157 14.933 /
\plot 13.157 14.933 13.098 14.922 /
\plot 13.098 14.922 13.032 14.912 /
\plot 13.032 14.912 12.967 14.901 /
\plot 12.967 14.901 12.903 14.891 /
\plot 12.903 14.891 12.838 14.880 /
\plot 12.838 14.880 12.772 14.870 /
\plot 12.772 14.870 12.706 14.857 /
\plot 12.706 14.857 12.639 14.844 /
\plot 12.639 14.844 12.571 14.831 /
\plot 12.571 14.831 12.503 14.819 /
\plot 12.503 14.819 12.435 14.806 /
\plot 12.435 14.806 12.366 14.791 /
\plot 12.366 14.791 12.298 14.776 /
\plot 12.298 14.776 12.228 14.762 /
\plot 12.228 14.762 12.158 14.745 /
\plot 12.158 14.745 12.090 14.730 /
\plot 12.090 14.730 12.023 14.713 /
\plot 12.023 14.713 11.955 14.694 /
\plot 11.955 14.694 11.889 14.677 /
\plot 11.889 14.677 11.826 14.658 /
\plot 11.826 14.658 11.762 14.639 /
\plot 11.762 14.639 11.699 14.620 /
\plot 11.699 14.620 11.637 14.601 /
\plot 11.637 14.601 11.578 14.582 /
\plot 11.578 14.582 11.521 14.561 /
\plot 11.521 14.561 11.464 14.539 /
\plot 11.464 14.539 11.407 14.518 /
\plot 11.407 14.518 11.352 14.495 /
\plot 11.352 14.495 11.299 14.472 /
\plot 11.299 14.472 11.246 14.450 /
\plot 11.246 14.450 11.195 14.427 /
\plot 11.195 14.427 11.144 14.404 /
\plot 11.144 14.404 11.093 14.379 /
\plot 11.093 14.379 11.041 14.351 /
\plot 11.041 14.351 10.988 14.323 /
\plot 10.988 14.323 10.935 14.294 /
\plot 10.935 14.294 10.880 14.262 /
\plot 10.880 14.262 10.827 14.230 /
\plot 10.827 14.230 10.772 14.196 /
\plot 10.772 14.196 10.715 14.163 /
\plot 10.715 14.163 10.660 14.127 /
\plot 10.660 14.127 10.605 14.089 /
\plot 10.605 14.089 10.547 14.048 /
\plot 10.547 14.048 10.492 14.008 /
\plot 10.492 14.008 10.437 13.968 /
\plot 10.437 13.968 10.382 13.926 /
\plot 10.382 13.926 10.327 13.883 /
\plot 10.327 13.883 10.274 13.839 /
\plot 10.274 13.839 10.224 13.796 /
\plot 10.224 13.796 10.171 13.752 /
\plot 10.171 13.752 10.122 13.705 /
\plot 10.122 13.705 10.073 13.661 /
\plot 10.073 13.661 10.025 13.617 /
\plot 10.025 13.617  9.980 13.570 /
\plot  9.980 13.570  9.934 13.523 /
\plot  9.934 13.523  9.889 13.477 /
\plot  9.889 13.477  9.847 13.430 /
\plot  9.847 13.430  9.804 13.384 /
\plot  9.804 13.384  9.764 13.335 /
\plot  9.764 13.335  9.724 13.288 /
\plot  9.724 13.288  9.686 13.242 /
\plot  9.686 13.242  9.648 13.193 /
\plot  9.648 13.193  9.610 13.144 /
\plot  9.610 13.144  9.572 13.094 /
\plot  9.572 13.094  9.533 13.043 /
\plot  9.533 13.043  9.495 12.988 /
\plot  9.495 12.988  9.455 12.933 /
\plot  9.455 12.933  9.415 12.878 /
\plot  9.415 12.878  9.377 12.821 /
\plot  9.377 12.821  9.337 12.761 /
\plot  9.337 12.761  9.296 12.702 /
\plot  9.296 12.702  9.256 12.641 /
\plot  9.256 12.641  9.216 12.579 /
\plot  9.216 12.579  9.176 12.518 /
\plot  9.176 12.518  9.136 12.454 /
\plot  9.136 12.454  9.095 12.391 /
\plot  9.095 12.391  9.055 12.330 /
\plot  9.055 12.330  9.017 12.268 /
\plot  9.017 12.268  8.977 12.205 /
\plot  8.977 12.205  8.939 12.143 /
\plot  8.939 12.143  8.901 12.084 /
\plot  8.901 12.084  8.862 12.025 /
\plot  8.862 12.025  8.827 11.966 /
\plot  8.827 11.966  8.788 11.908 /
\plot  8.788 11.908  8.752 11.851 /
\plot  8.752 11.851  8.719 11.796 /
\plot  8.719 11.796  8.683 11.741 /
\plot  8.683 11.741  8.649 11.688 /
\plot  8.649 11.688  8.615 11.637 /
\plot  8.615 11.637  8.581 11.587 /
\plot  8.581 11.587  8.547 11.536 /
\plot  8.547 11.536  8.507 11.479 /
\plot  8.507 11.479  8.467 11.422 /
\plot  8.467 11.422  8.426 11.366 /
\plot  8.426 11.366  8.386 11.309 /
\plot  8.386 11.309  8.344 11.254 /
\plot  8.344 11.254  8.302 11.197 /
\plot  8.302 11.197  8.259 11.142 /
\plot  8.259 11.142  8.215 11.085 /
\plot  8.215 11.085  8.170 11.028 /
\plot  8.170 11.028  8.124 10.973 /
\plot  8.124 10.973  8.077 10.916 /
\plot  8.077 10.916  8.029 10.861 /
\plot  8.029 10.861  7.982 10.806 /
\plot  7.982 10.806  7.933 10.753 /
\plot  7.933 10.753  7.887 10.700 /
\plot  7.887 10.700  7.838 10.649 /
\plot  7.838 10.649  7.789 10.598 /
\plot  7.789 10.598  7.743 10.549 /
\plot  7.743 10.549  7.696 10.503 /
\plot  7.696 10.503  7.650 10.458 /
\plot  7.650 10.458  7.603 10.414 /
\plot  7.603 10.414  7.559 10.374 /
\plot  7.559 10.374  7.514 10.334 /
\plot  7.514 10.334  7.472 10.295 /
\plot  7.472 10.295  7.427 10.259 /
\plot  7.427 10.259  7.385 10.226 /
\plot  7.385 10.226  7.345 10.192 /
\plot  7.345 10.192  7.303 10.160 /
\plot  7.303 10.160  7.254 10.124 /
\plot  7.254 10.124  7.205 10.090 /
\plot  7.205 10.090  7.156 10.056 /
\plot  7.156 10.056  7.106 10.025 /
\plot  7.106 10.025  7.055  9.993 /
\plot  7.055  9.993  7.002  9.963 /
\plot  7.002  9.963  6.949  9.934 /
\plot  6.949  9.934  6.894  9.906 /
\plot  6.894  9.906  6.841  9.881 /
\plot  6.841  9.881  6.786  9.855 /
\plot  6.786  9.855  6.731  9.832 /
\plot  6.731  9.832  6.674  9.811 /
\plot  6.674  9.811  6.621  9.792 /
\plot  6.621  9.792  6.566  9.775 /
\plot  6.566  9.775  6.513  9.758 /
\plot  6.513  9.758  6.460  9.745 /
\plot  6.460  9.745  6.407  9.735 /
\plot  6.407  9.735  6.358  9.724 /
\plot  6.358  9.724  6.310  9.718 /
\plot  6.310  9.718  6.263  9.711 /
\plot  6.263  9.711  6.217  9.709 /
\plot  6.217  9.709  6.172  9.707 /
\plot  6.172  9.707  6.128  9.707 /
\plot  6.128  9.707  6.085  9.709 /
\plot  6.085  9.709  6.039  9.716 /
\plot  6.039  9.716  5.994  9.722 /
\plot  5.994  9.722  5.948  9.730 /
\plot  5.948  9.730  5.901  9.743 /
\plot  5.901  9.743  5.853  9.758 /
\plot  5.853  9.758  5.802  9.775 /
\plot  5.802  9.775  5.749  9.796 /
\plot  5.749  9.796  5.692  9.821 /
\plot  5.692  9.821  5.632  9.849 /
\plot  5.632  9.849  5.569  9.881 /
\plot  5.569  9.881  5.503  9.914 /
\plot  5.503  9.914  5.438  9.950 /
\plot  5.438  9.950  5.370  9.989 /
\plot  5.370  9.989  5.306 10.025 /
\plot  5.306 10.025  5.247 10.061 /
\plot  5.247 10.061  5.194 10.090 /
\plot  5.194 10.090  5.152 10.116 /
\plot  5.152 10.116  5.120 10.137 /
\plot  5.120 10.137  5.097 10.149 /
\plot  5.097 10.149  5.086 10.156 /
\plot  5.086 10.156  5.080 10.160 /
}%
%  METADATA <id>6</id> 
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot 15.240 17.780 15.236 17.776 /
\plot 15.236 17.776 15.225 17.767 /
\plot 15.225 17.767 15.204 17.755 /
\plot 15.204 17.755 15.174 17.731 /
\plot 15.174 17.731 15.134 17.702 /
\plot 15.134 17.702 15.085 17.666 /
\plot 15.085 17.666 15.028 17.621 /
\plot 15.028 17.621 14.965 17.573 /
\plot 14.965 17.573 14.897 17.522 /
\plot 14.897 17.522 14.829 17.469 /
\plot 14.829 17.469 14.760 17.416 /
\plot 14.760 17.416 14.694 17.363 /
\plot 14.694 17.363 14.630 17.312 /
\plot 14.630 17.312 14.569 17.264 /
\plot 14.569 17.264 14.514 17.217 /
\plot 14.514 17.217 14.459 17.173 /
\plot 14.459 17.173 14.410 17.128 /
\plot 14.410 17.128 14.364 17.086 /
\plot 14.364 17.086 14.319 17.046 /
\plot 14.319 17.046 14.277 17.005 /
\plot 14.277 17.005 14.235 16.963 /
\plot 14.235 16.963 14.194 16.923 /
\plot 14.194 16.923 14.156 16.880 /
\plot 14.156 16.880 14.122 16.844 /
\plot 14.122 16.844 14.089 16.806 /
\plot 14.089 16.806 14.053 16.768 /
\plot 14.053 16.768 14.019 16.728 /
\plot 14.019 16.728 13.985 16.686 /
\plot 13.985 16.686 13.949 16.643 /
\plot 13.949 16.643 13.911 16.601 /
\plot 13.911 16.601 13.875 16.557 /
\plot 13.875 16.557 13.835 16.510 /
\plot 13.835 16.510 13.796 16.463 /
\plot 13.796 16.463 13.756 16.417 /
\plot 13.756 16.417 13.714 16.368 /
\plot 13.714 16.368 13.674 16.320 /
\plot 13.674 16.320 13.631 16.271 /
\plot 13.631 16.271 13.587 16.224 /
\plot 13.587 16.224 13.545 16.176 /
\plot 13.545 16.176 13.500 16.127 /
\plot 13.500 16.127 13.456 16.080 /
\plot 13.456 16.080 13.409 16.034 /
\plot 13.409 16.034 13.365 15.987 /
\plot 13.365 15.987 13.320 15.943 /
\plot 13.320 15.943 13.274 15.900 /
\plot 13.274 15.900 13.227 15.858 /
\plot 13.227 15.858 13.180 15.816 /
\plot 13.180 15.816 13.134 15.776 /
\plot 13.134 15.776 13.087 15.737 /
\plot 13.087 15.737 13.041 15.699 /
\plot 13.041 15.699 12.992 15.663 /
\plot 12.992 15.663 12.943 15.629 /
\plot 12.943 15.629 12.897 15.596 /
\plot 12.897 15.596 12.846 15.564 /
\plot 12.846 15.564 12.795 15.532 /
\plot 12.795 15.532 12.742 15.498 /
\plot 12.742 15.498 12.689 15.466 /
\plot 12.689 15.466 12.632 15.435 /
\plot 12.632 15.435 12.573 15.405 /
\plot 12.573 15.405 12.514 15.373 /
\plot 12.514 15.373 12.452 15.344 /
\plot 12.452 15.344 12.389 15.314 /
\plot 12.389 15.314 12.325 15.284 /
\plot 12.325 15.284 12.260 15.255 /
\plot 12.260 15.255 12.194 15.227 /
\plot 12.194 15.227 12.126 15.202 /
\plot 12.126 15.202 12.059 15.174 /
\plot 12.059 15.174 11.991 15.151 /
\plot 11.991 15.151 11.923 15.128 /
\plot 11.923 15.128 11.855 15.105 /
\plot 11.855 15.105 11.788 15.083 /
\plot 11.788 15.083 11.722 15.064 /
\plot 11.722 15.064 11.656 15.047 /
\plot 11.656 15.047 11.591 15.030 /
\plot 11.591 15.030 11.527 15.014 /
\plot 11.527 15.014 11.464 15.001 /
\plot 11.464 15.001 11.402 14.988 /
\plot 11.402 14.988 11.343 14.975 /
\plot 11.343 14.975 11.282 14.965 /
\plot 11.282 14.965 11.225 14.956 /
\plot 11.225 14.956 11.165 14.948 /
\plot 11.165 14.948 11.104 14.942 /
\plot 11.104 14.942 11.041 14.935 /
\plot 11.041 14.935 10.979 14.931 /
\plot 10.979 14.931 10.916 14.927 /
\plot 10.916 14.927 10.852 14.925 /
\plot 10.852 14.925 10.787 14.922 /
\plot 10.787 14.922 10.721 14.922 /
\plot 10.721 14.922 10.655 14.922 /
\plot 10.655 14.922 10.588 14.925 /
\plot 10.588 14.925 10.520 14.927 /
\plot 10.520 14.927 10.450 14.931 /
\plot 10.450 14.931 10.382 14.933 /
\plot 10.382 14.933 10.312 14.939 /
\plot 10.312 14.939 10.243 14.944 /
\plot 10.243 14.944 10.173 14.950 /
\plot 10.173 14.950 10.105 14.958 /
\plot 10.105 14.958 10.035 14.965 /
\plot 10.035 14.965  9.967 14.973 /
\plot  9.967 14.973  9.902 14.980 /
\plot  9.902 14.980  9.834 14.988 /
\plot  9.834 14.988  9.771 14.997 /
\plot  9.771 14.997  9.705 15.005 /
\plot  9.705 15.005  9.644 15.014 /
\plot  9.644 15.014  9.580 15.022 /
\plot  9.580 15.022  9.521 15.030 /
\plot  9.521 15.030  9.459 15.039 /
\plot  9.459 15.039  9.400 15.047 /
\plot  9.400 15.047  9.341 15.054 /
\plot  9.341 15.054  9.279 15.062 /
\plot  9.279 15.062  9.220 15.071 /
\plot  9.220 15.071  9.159 15.077 /
\plot  9.159 15.077  9.095 15.083 /
\plot  9.095 15.083  9.032 15.090 /
\plot  9.032 15.090  8.968 15.096 /
\plot  8.968 15.096  8.903 15.102 /
\plot  8.903 15.102  8.835 15.107 /
\plot  8.835 15.107  8.767 15.113 /
\plot  8.767 15.113  8.700 15.115 /
\plot  8.700 15.115  8.630 15.117 /
\plot  8.630 15.117  8.560 15.119 /
\plot  8.560 15.119  8.488 15.121 /
\plot  8.488 15.121  8.418 15.119 /
\plot  8.418 15.119  8.346 15.119 /
\plot  8.346 15.119  8.276 15.115 /
\plot  8.276 15.115  8.206 15.111 /
\plot  8.206 15.111  8.136 15.107 /
\plot  8.136 15.107  8.069 15.100 /
\plot  8.069 15.100  8.003 15.092 /
\plot  8.003 15.092  7.938 15.081 /
\plot  7.938 15.081  7.874 15.071 /
\plot  7.874 15.071  7.811 15.060 /
\plot  7.811 15.060  7.749 15.045 /
\plot  7.749 15.045  7.688 15.030 /
\plot  7.688 15.030  7.631 15.014 /
\plot  7.631 15.014  7.571 14.994 /
\plot  7.571 14.994  7.514 14.975 /
\plot  7.514 14.975  7.457 14.954 /
\plot  7.457 14.954  7.400 14.931 /
\plot  7.400 14.931  7.343 14.906 /
\plot  7.343 14.906  7.286 14.876 /
\plot  7.286 14.876  7.228 14.846 /
\plot  7.228 14.846  7.169 14.817 /
\plot  7.169 14.817  7.110 14.783 /
\plot  7.110 14.783  7.051 14.747 /
\plot  7.051 14.747  6.991 14.709 /
\plot  6.991 14.709  6.932 14.669 /
\plot  6.932 14.669  6.871 14.628 /
\plot  6.871 14.628  6.811 14.586 /
\plot  6.811 14.586  6.752 14.541 /
\plot  6.752 14.541  6.693 14.497 /
\plot  6.693 14.497  6.636 14.450 /
\plot  6.636 14.450  6.579 14.404 /
\plot  6.579 14.404  6.521 14.357 /
\plot  6.521 14.357  6.466 14.311 /
\plot  6.466 14.311  6.414 14.262 /
\plot  6.414 14.262  6.361 14.216 /
\plot  6.361 14.216  6.312 14.171 /
\plot  6.312 14.171  6.263 14.125 /
\plot  6.263 14.125  6.217 14.080 /
\plot  6.217 14.080  6.172 14.036 /
\plot  6.172 14.036  6.128 13.991 /
\plot  6.128 13.991  6.085 13.949 /
\plot  6.085 13.949  6.045 13.906 /
\plot  6.045 13.906  6.007 13.864 /
\plot  6.007 13.864  5.965 13.820 /
\plot  5.965 13.820  5.925 13.775 /
\plot  5.925 13.775  5.884 13.731 /
\plot  5.884 13.731  5.844 13.686 /
\plot  5.844 13.686  5.804 13.640 /
\plot  5.804 13.640  5.764 13.591 /
\plot  5.764 13.591  5.723 13.542 /
\plot  5.723 13.542  5.681 13.492 /
\plot  5.681 13.492  5.639 13.437 /
\plot  5.639 13.437  5.592 13.379 /
\plot  5.592 13.379  5.546 13.320 /
\plot  5.546 13.320  5.497 13.257 /
\plot  5.497 13.257  5.448 13.193 /
\plot  5.448 13.193  5.400 13.128 /
\plot  5.400 13.128  5.349 13.062 /
\plot  5.349 13.062  5.300 12.998 /
\plot  5.300 12.998  5.256 12.937 /
\plot  5.256 12.937  5.213 12.880 /
\plot  5.213 12.880  5.175 12.829 /
\plot  5.175 12.829  5.143 12.787 /
\plot  5.143 12.787  5.118 12.753 /
\plot  5.118 12.753  5.101 12.730 /
\plot  5.101 12.730  5.088 12.713 /
\plot  5.088 12.713  5.082 12.704 /
\plot  5.082 12.704  5.080 12.700 /
}%
%  METADATA <id>7</id> 
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
\setsolid
{\color[rgb]{0,0,0}\plot  5.080 12.700  5.082 12.702 /
\plot  5.082 12.702  5.091 12.708 /
\plot  5.091 12.708  5.103 12.721 /
\plot  5.103 12.721  5.122 12.738 /
\plot  5.122 12.738  5.150 12.761 /
\plot  5.150 12.761  5.186 12.791 /
\plot  5.186 12.791  5.228 12.827 /
\plot  5.228 12.827  5.277 12.867 /
\plot  5.277 12.867  5.330 12.912 /
\plot  5.330 12.912  5.387 12.958 /
\plot  5.387 12.958  5.446 13.005 /
\plot  5.446 13.005  5.508 13.051 /
\plot  5.508 13.051  5.569 13.096 /
\plot  5.569 13.096  5.630 13.140 /
\plot  5.630 13.140  5.692 13.183 /
\plot  5.692 13.183  5.753 13.223 /
\plot  5.753 13.223  5.814 13.261 /
\plot  5.814 13.261  5.876 13.297 /
\plot  5.876 13.297  5.937 13.331 /
\plot  5.937 13.331  6.001 13.365 /
\plot  6.001 13.365  6.064 13.396 /
\plot  6.064 13.396  6.132 13.428 /
\plot  6.132 13.428  6.200 13.460 /
\plot  6.200 13.460  6.274 13.490 /
\plot  6.274 13.490  6.350 13.519 /
\plot  6.350 13.519  6.401 13.540 /
\plot  6.401 13.540  6.456 13.561 /
\plot  6.456 13.561  6.511 13.581 /
\plot  6.511 13.581  6.568 13.602 /
\plot  6.568 13.602  6.627 13.623 /
\plot  6.627 13.623  6.689 13.644 /
\plot  6.689 13.644  6.752 13.665 /
\plot  6.752 13.665  6.820 13.686 /
\plot  6.820 13.686  6.888 13.710 /
\plot  6.888 13.710  6.957 13.733 /
\plot  6.957 13.733  7.032 13.754 /
\plot  7.032 13.754  7.106 13.777 /
\plot  7.106 13.777  7.184 13.803 /
\plot  7.184 13.803  7.264 13.826 /
\plot  7.264 13.826  7.345 13.849 /
\plot  7.345 13.849  7.430 13.875 /
\plot  7.430 13.875  7.514 13.898 /
\plot  7.514 13.898  7.601 13.923 /
\plot  7.601 13.923  7.690 13.949 /
\plot  7.690 13.949  7.781 13.974 /
\plot  7.781 13.974  7.872 14.000 /
\plot  7.872 14.000  7.963 14.023 /
\plot  7.963 14.023  8.056 14.048 /
\plot  8.056 14.048  8.149 14.074 /
\plot  8.149 14.074  8.242 14.099 /
\plot  8.242 14.099  8.338 14.125 /
\plot  8.338 14.125  8.431 14.148 /
\plot  8.431 14.148  8.526 14.173 /
\plot  8.526 14.173  8.619 14.196 /
\plot  8.619 14.196  8.714 14.220 /
\plot  8.714 14.220  8.807 14.243 /
\plot  8.807 14.243  8.901 14.268 /
\plot  8.901 14.268  8.992 14.290 /
\plot  8.992 14.290  9.085 14.313 /
\plot  9.085 14.313  9.176 14.336 /
\plot  9.176 14.336  9.267 14.357 /
\plot  9.267 14.357  9.358 14.381 /
\plot  9.358 14.381  9.449 14.402 /
\plot  9.449 14.402  9.540 14.425 /
\plot  9.540 14.425  9.631 14.446 /
\plot  9.631 14.446  9.718 14.467 /
\plot  9.718 14.467  9.804 14.489 /
\plot  9.804 14.489  9.893 14.510 /
\plot  9.893 14.510  9.982 14.531 /
\plot  9.982 14.531 10.071 14.552 /
\plot 10.071 14.552 10.162 14.573 /
\plot 10.162 14.573 10.253 14.594 /
\plot 10.253 14.594 10.346 14.618 /
\plot 10.346 14.618 10.439 14.639 /
\plot 10.439 14.639 10.535 14.662 /
\plot 10.535 14.662 10.630 14.685 /
\plot 10.630 14.685 10.727 14.709 /
\plot 10.727 14.709 10.825 14.734 /
\plot 10.825 14.734 10.922 14.757 /
\plot 10.922 14.757 11.021 14.783 /
\plot 11.021 14.783 11.119 14.808 /
\plot 11.119 14.808 11.218 14.834 /
\plot 11.218 14.834 11.318 14.859 /
\plot 11.318 14.859 11.417 14.884 /
\plot 11.417 14.884 11.515 14.910 /
\plot 11.515 14.910 11.614 14.937 /
\plot 11.614 14.937 11.712 14.963 /
\plot 11.712 14.963 11.807 14.990 /
\plot 11.807 14.990 11.902 15.018 /
\plot 11.902 15.018 11.997 15.045 /
\plot 11.997 15.045 12.088 15.071 /
\plot 12.088 15.071 12.181 15.098 /
\plot 12.181 15.098 12.270 15.126 /
\plot 12.270 15.126 12.357 15.153 /
\plot 12.357 15.153 12.444 15.181 /
\plot 12.444 15.181 12.526 15.206 /
\plot 12.526 15.206 12.609 15.234 /
\plot 12.609 15.234 12.687 15.261 /
\plot 12.687 15.261 12.766 15.289 /
\plot 12.766 15.289 12.840 15.314 /
\plot 12.840 15.314 12.914 15.342 /
\plot 12.914 15.342 12.984 15.369 /
\plot 12.984 15.369 13.051 15.395 /
\plot 13.051 15.395 13.119 15.422 /
\plot 13.119 15.422 13.185 15.450 /
\plot 13.185 15.450 13.246 15.477 /
\plot 13.246 15.477 13.310 15.505 /
\plot 13.310 15.505 13.392 15.543 /
\plot 13.392 15.543 13.473 15.583 /
\plot 13.473 15.583 13.551 15.625 /
\plot 13.551 15.625 13.629 15.665 /
\plot 13.629 15.665 13.703 15.710 /
\plot 13.703 15.710 13.775 15.754 /
\plot 13.775 15.754 13.847 15.799 /
\plot 13.847 15.799 13.917 15.845 /
\plot 13.917 15.845 13.985 15.892 /
\plot 13.985 15.892 14.050 15.941 /
\plot 14.050 15.941 14.116 15.989 /
\plot 14.116 15.989 14.177 16.040 /
\plot 14.177 16.040 14.237 16.091 /
\plot 14.237 16.091 14.296 16.142 /
\plot 14.296 16.142 14.351 16.192 /
\plot 14.351 16.192 14.404 16.243 /
\plot 14.404 16.243 14.455 16.294 /
\plot 14.455 16.294 14.503 16.345 /
\plot 14.503 16.345 14.548 16.396 /
\plot 14.548 16.396 14.590 16.444 /
\plot 14.590 16.444 14.633 16.493 /
\plot 14.633 16.493 14.669 16.540 /
\plot 14.669 16.540 14.704 16.586 /
\plot 14.704 16.586 14.738 16.631 /
\plot 14.738 16.631 14.768 16.675 /
\plot 14.768 16.675 14.798 16.720 /
\plot 14.798 16.720 14.825 16.760 /
\plot 14.825 16.760 14.851 16.802 /
\plot 14.851 16.802 14.874 16.842 /
\plot 14.874 16.842 14.897 16.880 /
\plot 14.897 16.880 14.925 16.933 /
\plot 14.925 16.933 14.952 16.984 /
\plot 14.952 16.984 14.975 17.035 /
\plot 14.975 17.035 14.999 17.088 /
\plot 14.999 17.088 15.022 17.141 /
\plot 15.022 17.141 15.043 17.194 /
\plot 15.043 17.194 15.062 17.251 /
\plot 15.062 17.251 15.083 17.310 /
\plot 15.083 17.310 15.102 17.374 /
\plot 15.102 17.374 15.121 17.437 /
\plot 15.121 17.437 15.138 17.505 /
\plot 15.138 17.505 15.157 17.575 /
\plot 15.157 17.575 15.174 17.642 /
\plot 15.174 17.642 15.189 17.708 /
\plot 15.189 17.708 15.204 17.769 /
\plot 15.204 17.769 15.215 17.822 /
\plot 15.215 17.822 15.225 17.867 /
\plot 15.225 17.867 15.232 17.899 /
\plot 15.232 17.899 15.236 17.922 /
\plot 15.236 17.922 15.238 17.932 /
\plot 15.238 17.932 15.240 17.939 /
}%
%  METADATA <id>8</id> 
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\putrule from 15.240 15.240 to 15.236 15.240
\putrule from 15.236 15.240 to 15.227 15.240
\plot 15.227 15.240 15.208 15.238 /
\plot 15.208 15.238 15.183 15.236 /
\plot 15.183 15.236 15.145 15.234 /
\plot 15.145 15.234 15.094 15.229 /
\plot 15.094 15.229 15.033 15.225 /
\plot 15.033 15.225 14.958 15.219 /
\plot 14.958 15.219 14.874 15.212 /
\plot 14.874 15.212 14.781 15.206 /
\plot 14.781 15.206 14.679 15.198 /
\plot 14.679 15.198 14.571 15.189 /
\plot 14.571 15.189 14.461 15.181 /
\plot 14.461 15.181 14.347 15.172 /
\plot 14.347 15.172 14.232 15.162 /
\plot 14.232 15.162 14.120 15.153 /
\plot 14.120 15.153 14.008 15.143 /
\plot 14.008 15.143 13.898 15.134 /
\plot 13.898 15.134 13.792 15.124 /
\plot 13.792 15.124 13.691 15.113 /
\plot 13.691 15.113 13.593 15.105 /
\plot 13.593 15.105 13.498 15.094 /
\plot 13.498 15.094 13.407 15.085 /
\plot 13.407 15.085 13.320 15.075 /
\plot 13.320 15.075 13.236 15.064 /
\plot 13.236 15.064 13.153 15.054 /
\plot 13.153 15.054 13.075 15.045 /
\plot 13.075 15.045 12.996 15.035 /
\plot 12.996 15.035 12.920 15.022 /
\plot 12.920 15.022 12.844 15.011 /
\plot 12.844 15.011 12.770 15.001 /
\plot 12.770 15.001 12.696 14.988 /
\plot 12.696 14.988 12.622 14.975 /
\plot 12.622 14.975 12.554 14.963 /
\plot 12.554 14.963 12.486 14.952 /
\plot 12.486 14.952 12.416 14.939 /
\plot 12.416 14.939 12.349 14.927 /
\plot 12.349 14.927 12.279 14.912 /
\plot 12.279 14.912 12.207 14.897 /
\plot 12.207 14.897 12.135 14.882 /
\plot 12.135 14.882 12.061 14.867 /
\plot 12.061 14.867 11.985 14.853 /
\plot 11.985 14.853 11.908 14.836 /
\plot 11.908 14.836 11.832 14.819 /
\plot 11.832 14.819 11.754 14.800 /
\plot 11.754 14.800 11.673 14.781 /
\plot 11.673 14.781 11.593 14.762 /
\plot 11.593 14.762 11.510 14.743 /
\plot 11.510 14.743 11.428 14.721 /
\plot 11.428 14.721 11.345 14.702 /
\plot 11.345 14.702 11.261 14.681 /
\plot 11.261 14.681 11.178 14.658 /
\plot 11.178 14.658 11.093 14.637 /
\plot 11.093 14.637 11.009 14.613 /
\plot 11.009 14.613 10.924 14.592 /
\plot 10.924 14.592 10.839 14.569 /
\plot 10.839 14.569 10.757 14.546 /
\plot 10.757 14.546 10.672 14.522 /
\plot 10.672 14.522 10.590 14.497 /
\plot 10.590 14.497 10.509 14.474 /
\plot 10.509 14.474 10.427 14.450 /
\plot 10.427 14.450 10.346 14.427 /
\plot 10.346 14.427 10.268 14.402 /
\plot 10.268 14.402 10.190 14.379 /
\plot 10.190 14.379 10.111 14.355 /
\plot 10.111 14.355 10.033 14.330 /
\plot 10.033 14.330  9.957 14.307 /
\plot  9.957 14.307  9.883 14.281 /
\plot  9.883 14.281  9.807 14.258 /
\plot  9.807 14.258  9.732 14.232 /
\plot  9.732 14.232  9.658 14.207 /
\plot  9.658 14.207  9.578 14.182 /
\plot  9.578 14.182  9.500 14.154 /
\plot  9.500 14.154  9.419 14.127 /
\plot  9.419 14.127  9.339 14.099 /
\plot  9.339 14.099  9.258 14.072 /
\plot  9.258 14.072  9.176 14.042 /
\plot  9.176 14.042  9.093 14.012 /
\plot  9.093 14.012  9.009 13.983 /
\plot  9.009 13.983  8.924 13.951 /
\plot  8.924 13.951  8.837 13.919 /
\plot  8.837 13.919  8.752 13.887 /
\plot  8.752 13.887  8.664 13.856 /
\plot  8.664 13.856  8.577 13.822 /
\plot  8.577 13.822  8.490 13.788 /
\plot  8.490 13.788  8.401 13.754 /
\plot  8.401 13.754  8.314 13.720 /
\plot  8.314 13.720  8.227 13.686 /
\plot  8.227 13.686  8.141 13.653 /
\plot  8.141 13.653  8.054 13.619 /
\plot  8.054 13.619  7.969 13.585 /
\plot  7.969 13.585  7.887 13.551 /
\plot  7.887 13.551  7.804 13.517 /
\plot  7.804 13.517  7.722 13.483 /
\plot  7.722 13.483  7.643 13.449 /
\plot  7.643 13.449  7.567 13.418 /
\plot  7.567 13.418  7.491 13.386 /
\plot  7.491 13.386  7.419 13.354 /
\plot  7.419 13.354  7.347 13.322 /
\plot  7.347 13.322  7.277 13.293 /
\plot  7.277 13.293  7.211 13.263 /
\plot  7.211 13.263  7.146 13.233 /
\plot  7.146 13.233  7.084 13.206 /
\plot  7.084 13.206  7.023 13.178 /
\plot  7.023 13.178  6.966 13.151 /
\plot  6.966 13.151  6.909 13.123 /
\plot  6.909 13.123  6.854 13.096 /
\plot  6.854 13.096  6.778 13.060 /
\plot  6.778 13.060  6.706 13.026 /
\plot  6.706 13.026  6.636 12.990 /
\plot  6.636 12.990  6.568 12.954 /
\plot  6.568 12.954  6.500 12.918 /
\plot  6.500 12.918  6.435 12.882 /
\plot  6.435 12.882  6.371 12.846 /
\plot  6.371 12.846  6.308 12.810 /
\plot  6.308 12.810  6.248 12.774 /
\plot  6.248 12.774  6.189 12.738 /
\plot  6.189 12.738  6.132 12.700 /
\plot  6.132 12.700  6.075 12.664 /
\plot  6.075 12.664  6.022 12.628 /
\plot  6.022 12.628  5.971 12.592 /
\plot  5.971 12.592  5.925 12.556 /
\plot  5.925 12.556  5.878 12.520 /
\plot  5.878 12.520  5.836 12.486 /
\plot  5.836 12.486  5.795 12.452 /
\plot  5.795 12.452  5.757 12.418 /
\plot  5.757 12.418  5.721 12.385 /
\plot  5.721 12.385  5.690 12.353 /
\plot  5.690 12.353  5.658 12.321 /
\plot  5.658 12.321  5.630 12.289 /
\plot  5.630 12.289  5.605 12.260 /
\plot  5.605 12.260  5.580 12.228 /
\plot  5.580 12.228  5.556 12.196 /
\plot  5.556 12.196  5.529 12.156 /
\plot  5.529 12.156  5.501 12.116 /
\plot  5.501 12.116  5.478 12.073 /
\plot  5.478 12.073  5.455 12.031 /
\plot  5.455 12.031  5.431 11.985 /
\plot  5.431 11.985  5.410 11.938 /
\plot  5.410 11.938  5.391 11.891 /
\plot  5.391 11.891  5.372 11.841 /
\plot  5.372 11.841  5.355 11.792 /
\plot  5.355 11.792  5.340 11.741 /
\plot  5.340 11.741  5.326 11.688 /
\plot  5.326 11.688  5.313 11.637 /
\plot  5.313 11.637  5.300 11.587 /
\plot  5.300 11.587  5.290 11.536 /
\plot  5.290 11.536  5.279 11.485 /
\plot  5.279 11.485  5.271 11.436 /
\plot  5.271 11.436  5.262 11.388 /
\plot  5.262 11.388  5.254 11.339 /
\plot  5.254 11.339  5.245 11.292 /
\plot  5.245 11.292  5.239 11.244 /
\plot  5.239 11.244  5.232 11.201 /
\plot  5.232 11.201  5.226 11.157 /
\plot  5.226 11.157  5.218 11.113 /
\plot  5.218 11.113  5.211 11.066 /
\plot  5.211 11.066  5.205 11.015 /
\plot  5.205 11.015  5.196 10.962 /
\plot  5.196 10.962  5.188 10.907 /
\plot  5.188 10.907  5.179 10.846 /
\plot  5.179 10.846  5.169 10.780 /
\plot  5.169 10.780  5.160 10.712 /
\plot  5.160 10.712  5.150 10.640 /
\plot  5.150 10.640  5.139 10.564 /
\plot  5.139 10.564  5.127 10.490 /
\plot  5.127 10.490  5.118 10.418 /
\plot  5.118 10.418  5.108 10.351 /
\plot  5.108 10.351  5.099 10.291 /
\plot  5.099 10.291  5.093 10.243 /
\plot  5.093 10.243  5.086 10.204 /
\plot  5.086 10.204  5.082 10.181 /
\plot  5.082 10.181  5.080 10.166 /
\putrule from  5.080 10.166 to  5.080 10.160
}%
%  METADATA <id>18</id> 
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  5.112 11.430  6.636  9.874 /
}%
%  METADATA <id>19</id> 
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  5.112 12.732  7.398 10.382 /
}%
%  METADATA <id>20</id> 
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  5.620 13.399  8.064 11.081 /
}%
%  METADATA <id>21</id> 
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  6.223 14.097  8.604 11.811 /
}%
%  METADATA <id>22</id> 
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  6.890 14.637  9.049 12.541 /
}%
%  METADATA <id>23</id> 
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  7.715 15.081  9.652 13.272 /
}%
%  METADATA <id>28</id> 
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot 12.522 15.369 12.975 14.956 /
}%
%  METADATA <id>29</id> 
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot 13.193 15.903 13.942 15.153 /
}%
%  METADATA <id>30</id> 
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot 13.843 16.612 15.145 15.291 /
}%
%  METADATA <id>31</id> 
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot 14.417 17.185 15.204 16.514 /
}%
%  METADATA <id>32</id> 
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  9.131 15.035 10.234 13.851 /
}%
%  METADATA <id>33</id> 
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot 10.433 14.916 11.024 14.385 /
}%
%  METADATA <id>34</id> 
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot 11.557 15.035 11.891 14.719 /
}%
%  METADATA <id>9</id> 
%
% Fig TEXT object
%
\put{\SetFigFont{6}{7.2}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\Ga_u$}%
} [lB] at  8.350 15.240
%  METADATA <id>10</id> 
%
% Fig TEXT object
%
\put{\SetFigFont{6}{7.2}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\Ga_d$}%
} [lB] at  9.652 12.764
%  METADATA <id>11</id> 
%
% Fig TEXT object
%
\put{\SetFigFont{6}{7.2}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\tilde{S}_-$}%
} [lB] at  3.842 12.637
%  METADATA <id>12</id> 
%
% Fig TEXT object
%
\put{\SetFigFont{6}{7.2}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\bar{N}_-$}%
} [lB] at  3.873 10.160
%  METADATA <id>13</id> 
%
% Fig TEXT object
%
\put{\SetFigFont{6}{7.2}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\bar{N}_+$}%
} [lB] at 15.335 17.780
%  METADATA <id>14</id> 
%
% Fig TEXT object
%
\put{\SetFigFont{6}{7.2}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\tilde{S}_+$}%
} [lB] at 15.526 15.304
%  METADATA <id>15</id> 
%
% Fig TEXT object
%
\put{\SetFigFont{6}{7.2}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\cN$}%
} [lB] at  9.620 18.605
%  METADATA <id>16</id> 
%
% Fig TEXT object
%
\put{\SetFigFont{6}{7.2}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\cP$}%
} [lB] at  7.271 12.478
%  METADATA <id>17</id> 
%
% Fig TEXT object
%
\put{\SetFigFont{6}{7.2}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\cN$}%
} [lB] at 12.668 12.827
\linethickness=0pt
\putrectangle corners at  3.810 21.660 and 15.558  6.280
\endpicture}


==> KTZ_zGKN_I_thcor1.tex <==
%Title: /tmp/xfig-fig007472
%%Created by: fig2dev Version 3.2 Patchlevel 5
%%CreationDate: Wed Feb 18 13:00:43 1970
%%User: shadi@attar (Tahvildar-Zadeh A. Shadi)
\font\thinlinefont=cmr5
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\mbox{\beginpicture
\setcoordinatesystem units <0.50000cm,0.50000cm>
\unitlength=0.50000cm
\linethickness=1pt
\setplotsymbol ({\makebox(0,0)[l]{\tencirc\symbol{'160}}})
\setshadesymbol ({\thinlinefont .})
\setlinear
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\putrule from  5.080 16.510 to 15.240 16.510
}%
%
% Fig POLYLINE object
%
\linethickness=1pt
\setplotsymbol ({\makebox(0,0)[l]{\tencirc\symbol{'160}}})
{\color[rgb]{0,0,0}\putrule from  5.080 21.590 to 15.240 21.590
}%
%
% Fig POLYLINE object
%
\linethickness=1pt
\setplotsymbol ({\makebox(0,0)[l]{\tencirc\symbol{'160}}})
{\color[rgb]{0,0,0}\putrule from 15.240 21.590 to 15.240  6.315
\putrule from 15.240  6.350 to  5.045  6.350
\putrule from  5.080  6.350 to  5.080 21.590
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\putrule from  5.080 11.430 to 15.240 11.430
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  5.080 16.510 15.240 11.430 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  8.096 15.240  8.572 14.446 /
%
% arrow head
%
\plot  8.387 14.631  8.572 14.446  8.496 14.697 /
%
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot 11.748 13.335 12.224 12.700 /
%
% arrow head
%
\plot 12.021 12.865 12.224 12.700 12.122 12.941 /
%
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  5.080 16.510  5.082 16.506 /
\plot  5.082 16.506  5.086 16.493 /
\plot  5.086 16.493  5.093 16.474 /
\plot  5.093 16.474  5.103 16.442 /
\plot  5.103 16.442  5.118 16.398 /
\plot  5.118 16.398  5.137 16.343 /
\plot  5.137 16.343  5.160 16.277 /
\plot  5.160 16.277  5.186 16.201 /
\plot  5.186 16.201  5.215 16.116 /
\plot  5.215 16.116  5.245 16.025 /
\plot  5.245 16.025  5.277 15.932 /
\plot  5.277 15.932  5.309 15.839 /
\plot  5.309 15.839  5.338 15.744 /
\plot  5.338 15.744  5.368 15.653 /
\plot  5.368 15.653  5.395 15.564 /
\plot  5.395 15.564  5.423 15.477 /
\plot  5.423 15.477  5.448 15.397 /
\plot  5.448 15.397  5.472 15.318 /
\plot  5.472 15.318  5.493 15.244 /
\plot  5.493 15.244  5.512 15.174 /
\plot  5.512 15.174  5.529 15.107 /
\plot  5.529 15.107  5.546 15.041 /
\plot  5.546 15.041  5.560 14.978 /
\plot  5.560 14.978  5.573 14.916 /
\plot  5.573 14.916  5.586 14.857 /
\plot  5.586 14.857  5.599 14.798 /
\plot  5.599 14.798  5.609 14.736 /
\plot  5.609 14.736  5.620 14.677 /
\plot  5.620 14.677  5.628 14.618 /
\plot  5.628 14.618  5.637 14.556 /
\plot  5.637 14.556  5.645 14.493 /
\plot  5.645 14.493  5.654 14.431 /
\plot  5.654 14.431  5.660 14.366 /
\plot  5.660 14.366  5.666 14.300 /
\plot  5.666 14.300  5.671 14.235 /
\plot  5.671 14.235  5.675 14.167 /
\plot  5.675 14.167  5.679 14.097 /
\plot  5.679 14.097  5.681 14.029 /
\plot  5.681 14.029  5.683 13.959 /
\plot  5.683 13.959  5.685 13.890 /
\putrule from  5.685 13.890 to  5.685 13.818
\putrule from  5.685 13.818 to  5.685 13.748
\plot  5.685 13.748  5.683 13.680 /
\plot  5.683 13.680  5.681 13.610 /
\plot  5.681 13.610  5.679 13.542 /
\plot  5.679 13.542  5.675 13.477 /
\plot  5.675 13.477  5.671 13.411 /
\plot  5.671 13.411  5.666 13.346 /
\plot  5.666 13.346  5.660 13.284 /
\plot  5.660 13.284  5.654 13.223 /
\plot  5.654 13.223  5.645 13.164 /
\plot  5.645 13.164  5.637 13.106 /
\plot  5.637 13.106  5.628 13.049 /
\plot  5.628 13.049  5.620 12.992 /
\plot  5.620 12.992  5.609 12.937 /
\plot  5.609 12.937  5.599 12.880 /
\plot  5.599 12.880  5.586 12.821 /
\plot  5.586 12.821  5.571 12.764 /
\plot  5.571 12.764  5.556 12.704 /
\plot  5.556 12.704  5.539 12.645 /
\plot  5.539 12.645  5.520 12.581 /
\plot  5.520 12.581  5.501 12.518 /
\plot  5.501 12.518  5.480 12.450 /
\plot  5.480 12.450  5.455 12.380 /
\plot  5.455 12.380  5.429 12.306 /
\plot  5.429 12.306  5.400 12.230 /
\plot  5.400 12.230  5.370 12.150 /
\plot  5.370 12.150  5.338 12.067 /
\plot  5.338 12.067  5.304 11.982 /
\plot  5.304 11.982  5.273 11.898 /
\plot  5.273 11.898  5.239 11.813 /
\plot  5.239 11.813  5.207 11.735 /
\plot  5.207 11.735  5.175 11.661 /
\plot  5.175 11.661  5.150 11.597 /
\plot  5.150 11.597  5.127 11.542 /
\plot  5.127 11.542  5.110 11.498 /
\plot  5.110 11.498  5.095 11.468 /
\plot  5.095 11.468  5.086 11.447 /
\plot  5.086 11.447  5.082 11.434 /
\plot  5.082 11.434  5.080 11.430 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot 15.240 16.510 15.238 16.506 /
\plot 15.238 16.506 15.234 16.493 /
\plot 15.234 16.493 15.227 16.474 /
\plot 15.227 16.474 15.217 16.442 /
\plot 15.217 16.442 15.202 16.398 /
\plot 15.202 16.398 15.183 16.343 /
\plot 15.183 16.343 15.160 16.275 /
\plot 15.160 16.275 15.134 16.199 /
\plot 15.134 16.199 15.105 16.114 /
\plot 15.105 16.114 15.075 16.023 /
\plot 15.075 16.023 15.043 15.930 /
\plot 15.043 15.930 15.011 15.835 /
\plot 15.011 15.835 14.982 15.740 /
\plot 14.982 15.740 14.952 15.646 /
\plot 14.952 15.646 14.925 15.558 /
\plot 14.925 15.558 14.897 15.471 /
\plot 14.897 15.471 14.872 15.388 /
\plot 14.872 15.388 14.848 15.308 /
\plot 14.848 15.308 14.827 15.234 /
\plot 14.827 15.234 14.808 15.162 /
\plot 14.808 15.162 14.791 15.092 /
\plot 14.791 15.092 14.774 15.026 /
\plot 14.774 15.026 14.760 14.961 /
\plot 14.760 14.961 14.747 14.897 /
\plot 14.747 14.897 14.734 14.836 /
\plot 14.734 14.836 14.721 14.772 /
\plot 14.721 14.772 14.711 14.711 /
\plot 14.711 14.711 14.700 14.647 /
\plot 14.700 14.647 14.692 14.586 /
\plot 14.692 14.586 14.683 14.520 /
\plot 14.683 14.520 14.675 14.455 /
\plot 14.675 14.455 14.666 14.389 /
\plot 14.666 14.389 14.660 14.321 /
\plot 14.660 14.321 14.654 14.252 /
\plot 14.654 14.252 14.649 14.182 /
\plot 14.649 14.182 14.645 14.110 /
\plot 14.645 14.110 14.641 14.038 /
\plot 14.641 14.038 14.639 13.964 /
\plot 14.639 13.964 14.637 13.892 /
\plot 14.637 13.892 14.635 13.818 /
\putrule from 14.635 13.818 to 14.635 13.744
\putrule from 14.635 13.744 to 14.635 13.669
\plot 14.635 13.669 14.637 13.595 /
\plot 14.637 13.595 14.639 13.523 /
\plot 14.639 13.523 14.641 13.454 /
\plot 14.641 13.454 14.645 13.384 /
\plot 14.645 13.384 14.649 13.316 /
\plot 14.649 13.316 14.654 13.248 /
\plot 14.654 13.248 14.660 13.185 /
\plot 14.660 13.185 14.666 13.121 /
\plot 14.666 13.121 14.675 13.060 /
\plot 14.675 13.060 14.683 13.001 /
\plot 14.683 13.001 14.692 12.943 /
\plot 14.692 12.943 14.700 12.888 /
\plot 14.700 12.888 14.711 12.831 /
\plot 14.711 12.831 14.721 12.774 /
\plot 14.721 12.774 14.734 12.717 /
\plot 14.734 12.717 14.749 12.660 /
\plot 14.749 12.660 14.764 12.603 /
\plot 14.764 12.603 14.781 12.543 /
\plot 14.781 12.543 14.800 12.486 /
\plot 14.800 12.486 14.819 12.425 /
\plot 14.819 12.425 14.840 12.361 /
\plot 14.840 12.361 14.865 12.296 /
\plot 14.865 12.296 14.891 12.228 /
\plot 14.891 12.228 14.920 12.156 /
\plot 14.920 12.156 14.950 12.082 /
\plot 14.950 12.082 14.982 12.006 /
\plot 14.982 12.006 15.016 11.930 /
\plot 15.016 11.930 15.047 11.851 /
\plot 15.047 11.851 15.081 11.777 /
\plot 15.081 11.777 15.113 11.705 /
\plot 15.113 11.705 15.145 11.637 /
\plot 15.145 11.637 15.170 11.580 /
\plot 15.170 11.580 15.193 11.532 /
\plot 15.193 11.532 15.210 11.491 /
\plot 15.210 11.491 15.225 11.464 /
\plot 15.225 11.464 15.234 11.445 /
\plot 15.234 11.445 15.238 11.434 /
\plot 15.238 11.434 15.240 11.430 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  5.080 16.510  5.082 16.508 /
\plot  5.082 16.508  5.084 16.504 /
\plot  5.084 16.504  5.091 16.497 /
\plot  5.091 16.497  5.101 16.485 /
\plot  5.101 16.485  5.116 16.466 /
\plot  5.116 16.466  5.135 16.440 /
\plot  5.135 16.440  5.160 16.408 /
\plot  5.160 16.408  5.192 16.368 /
\plot  5.192 16.368  5.230 16.317 /
\plot  5.230 16.317  5.277 16.260 /
\plot  5.277 16.260  5.330 16.190 /
\plot  5.330 16.190  5.391 16.114 /
\plot  5.391 16.114  5.461 16.025 /
\plot  5.461 16.025  5.537 15.928 /
\plot  5.537 15.928  5.624 15.820 /
\plot  5.624 15.820  5.715 15.701 /
\plot  5.715 15.701  5.817 15.574 /
\plot  5.817 15.574  5.922 15.439 /
\plot  5.922 15.439  6.037 15.293 /
\plot  6.037 15.293  6.157 15.141 /
\plot  6.157 15.141  6.282 14.982 /
\plot  6.282 14.982  6.413 14.815 /
\plot  6.413 14.815  6.549 14.643 /
\plot  6.549 14.643  6.687 14.467 /
\plot  6.687 14.467  6.830 14.285 /
\plot  6.830 14.285  6.974 14.101 /
\plot  6.974 14.101  7.123 13.915 /
\plot  7.123 13.915  7.271 13.727 /
\plot  7.271 13.727  7.421 13.536 /
\plot  7.421 13.536  7.569 13.348 /
\plot  7.569 13.348  7.719 13.157 /
\plot  7.719 13.157  7.870 12.969 /
\plot  7.870 12.969  8.016 12.780 /
\plot  8.016 12.780  8.164 12.596 /
\plot  8.164 12.596  8.308 12.412 /
\plot  8.308 12.412  8.450 12.232 /
\plot  8.450 12.232  8.589 12.057 /
\plot  8.589 12.057  8.727 11.883 /
\plot  8.727 11.883  8.862 11.714 /
\plot  8.862 11.714  8.994 11.546 /
\plot  8.994 11.546  9.121 11.386 /
\plot  9.121 11.386  9.248 11.227 /
\plot  9.248 11.227  9.368 11.074 /
\plot  9.368 11.074  9.487 10.924 /
\plot  9.487 10.924  9.603 10.780 /
\plot  9.603 10.780  9.716 10.638 /
\plot  9.716 10.638  9.823 10.503 /
\plot  9.823 10.503  9.929 10.370 /
\plot  9.929 10.370 10.031 10.240 /
\plot 10.031 10.240 10.130 10.118 /
\plot 10.130 10.118 10.228  9.997 /
\plot 10.228  9.997 10.321  9.881 /
\plot 10.321  9.881 10.412  9.768 /
\plot 10.412  9.768 10.499  9.658 /
\plot 10.499  9.658 10.583  9.553 /
\plot 10.583  9.553 10.668  9.451 /
\plot 10.668  9.451 10.746  9.351 /
\plot 10.746  9.351 10.825  9.256 /
\plot 10.825  9.256 10.901  9.163 /
\plot 10.901  9.163 10.975  9.072 /
\plot 10.975  9.072 11.047  8.983 /
\plot 11.047  8.983 11.117  8.898 /
\plot 11.117  8.898 11.184  8.816 /
\plot 11.184  8.816 11.250  8.735 /
\plot 11.250  8.735 11.316  8.657 /
\plot 11.316  8.657 11.379  8.581 /
\plot 11.379  8.581 11.441  8.505 /
\plot 11.441  8.505 11.502  8.433 /
\plot 11.502  8.433 11.563  8.361 /
\plot 11.563  8.361 11.665  8.240 /
\plot 11.665  8.240 11.764  8.122 /
\plot 11.764  8.122 11.860  8.009 /
\plot 11.860  8.009 11.955  7.899 /
\plot 11.955  7.899 12.046  7.794 /
\plot 12.046  7.794 12.135  7.690 /
\plot 12.135  7.690 12.224  7.590 /
\plot 12.224  7.590 12.308  7.493 /
\plot 12.308  7.493 12.391  7.400 /
\plot 12.391  7.400 12.474  7.309 /
\plot 12.474  7.309 12.554  7.222 /
\plot 12.554  7.222 12.630  7.137 /
\plot 12.630  7.137 12.706  7.055 /
\plot 12.706  7.055 12.780  6.977 /
\plot 12.780  6.977 12.852  6.900 /
\plot 12.852  6.900 12.922  6.828 /
\plot 12.922  6.828 12.990  6.759 /
\plot 12.990  6.759 13.056  6.693 /
\plot 13.056  6.693 13.119  6.629 /
\plot 13.119  6.629 13.180  6.570 /
\plot 13.180  6.570 13.240  6.513 /
\plot 13.240  6.513 13.297  6.460 /
\plot 13.297  6.460 13.352  6.409 /
\plot 13.352  6.409 13.405  6.361 /
\plot 13.405  6.361 13.456  6.316 /
\plot 13.456  6.316 13.502  6.276 /
\plot 13.502  6.276 13.549  6.236 /
\plot 13.549  6.236 13.593  6.200 /
\plot 13.593  6.200 13.636  6.166 /
\plot 13.636  6.166 13.676  6.136 /
\plot 13.676  6.136 13.714  6.107 /
\plot 13.714  6.107 13.750  6.079 /
\plot 13.750  6.079 13.786  6.056 /
\plot 13.786  6.056 13.820  6.032 /
\plot 13.820  6.032 13.851  6.011 /
\plot 13.851  6.011 13.881  5.992 /
\plot 13.881  5.992 13.913  5.973 /
\plot 13.913  5.973 13.940  5.958 /
\plot 13.940  5.958 13.968  5.941 /
\plot 13.968  5.941 13.998  5.927 /
\plot 13.998  5.927 14.046  5.901 /
\plot 14.046  5.901 14.093  5.878 /
\plot 14.093  5.878 14.141  5.857 /
\plot 14.141  5.857 14.188  5.838 /
\plot 14.188  5.838 14.232  5.821 /
\plot 14.232  5.821 14.279  5.806 /
\plot 14.279  5.806 14.323  5.791 /
\plot 14.323  5.791 14.368  5.781 /
\plot 14.368  5.781 14.412  5.772 /
\plot 14.412  5.772 14.455  5.764 /
\plot 14.455  5.764 14.497  5.759 /
\plot 14.497  5.759 14.537  5.755 /
\putrule from 14.537  5.755 to 14.575  5.755
\putrule from 14.575  5.755 to 14.611  5.755
\plot 14.611  5.755 14.647  5.759 /
\plot 14.647  5.759 14.679  5.764 /
\plot 14.679  5.764 14.711  5.770 /
\plot 14.711  5.770 14.740  5.776 /
\plot 14.740  5.776 14.768  5.787 /
\plot 14.768  5.787 14.796  5.798 /
\plot 14.796  5.798 14.819  5.808 /
\plot 14.819  5.808 14.844  5.821 /
\plot 14.844  5.821 14.874  5.840 /
\plot 14.874  5.840 14.903  5.863 /
\plot 14.903  5.863 14.933  5.889 /
\plot 14.933  5.889 14.963  5.918 /
\plot 14.963  5.918 14.992  5.954 /
\plot 14.992  5.954 15.022  5.994 /
\plot 15.022  5.994 15.054  6.041 /
\plot 15.054  6.041 15.088  6.092 /
\plot 15.088  6.092 15.121  6.145 /
\plot 15.121  6.145 15.155  6.200 /
\plot 15.155  6.200 15.183  6.251 /
\plot 15.183  6.251 15.208  6.293 /
\plot 15.208  6.293 15.225  6.322 /
\plot 15.225  6.322 15.236  6.342 /
\plot 15.236  6.342 15.240  6.348 /
\putrule from 15.240  6.348 to 15.240  6.350
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot 15.240 11.430 15.238 11.432 /
\plot 15.238 11.432 15.236 11.436 /
\plot 15.236 11.436 15.229 11.445 /
\plot 15.229 11.445 15.219 11.458 /
\plot 15.219 11.458 15.206 11.479 /
\plot 15.206 11.479 15.187 11.504 /
\plot 15.187 11.504 15.162 11.540 /
\plot 15.162 11.540 15.130 11.582 /
\plot 15.130 11.582 15.094 11.635 /
\plot 15.094 11.635 15.050 11.697 /
\plot 15.050 11.697 14.997 11.769 /
\plot 14.997 11.769 14.937 11.853 /
\plot 14.937 11.853 14.872 11.946 /
\plot 14.872 11.946 14.796 12.050 /
\plot 14.796 12.050 14.715 12.164 /
\plot 14.715 12.164 14.626 12.287 /
\plot 14.626 12.287 14.531 12.421 /
\plot 14.531 12.421 14.427 12.565 /
\plot 14.427 12.565 14.319 12.715 /
\plot 14.319 12.715 14.205 12.874 /
\plot 14.205 12.874 14.086 13.039 /
\plot 14.086 13.039 13.964 13.212 /
\plot 13.964 13.212 13.835 13.390 /
\plot 13.835 13.390 13.703 13.572 /
\plot 13.703 13.572 13.570 13.758 /
\plot 13.570 13.758 13.434 13.947 /
\plot 13.434 13.947 13.297 14.137 /
\plot 13.297 14.137 13.159 14.330 /
\plot 13.159 14.330 13.020 14.522 /
\plot 13.020 14.522 12.882 14.715 /
\plot 12.882 14.715 12.744 14.906 /
\plot 12.744 14.906 12.607 15.096 /
\plot 12.607 15.096 12.471 15.284 /
\plot 12.471 15.284 12.338 15.469 /
\plot 12.338 15.469 12.205 15.653 /
\plot 12.205 15.653 12.076 15.831 /
\plot 12.076 15.831 11.949 16.006 /
\plot 11.949 16.006 11.824 16.180 /
\plot 11.824 16.180 11.701 16.347 /
\plot 11.701 16.347 11.582 16.510 /
\plot 11.582 16.510 11.466 16.669 /
\plot 11.466 16.669 11.354 16.825 /
\plot 11.354 16.825 11.244 16.976 /
\plot 11.244 16.976 11.138 17.122 /
\plot 11.138 17.122 11.034 17.264 /
\plot 11.034 17.264 10.933 17.399 /
\plot 10.933 17.399 10.835 17.532 /
\plot 10.835 17.532 10.740 17.661 /
\plot 10.740 17.661 10.649 17.786 /
\plot 10.649 17.786 10.560 17.907 /
\plot 10.560 17.907 10.473 18.023 /
\plot 10.473 18.023 10.389 18.136 /
\plot 10.389 18.136 10.308 18.246 /
\plot 10.308 18.246 10.230 18.351 /
\plot 10.230 18.351 10.152 18.453 /
\plot 10.152 18.453 10.077 18.553 /
\plot 10.077 18.553 10.005 18.648 /
\plot 10.005 18.648  9.934 18.741 /
\plot  9.934 18.741  9.866 18.832 /
\plot  9.866 18.832  9.798 18.919 /
\plot  9.798 18.919  9.732 19.006 /
\plot  9.732 19.006  9.669 19.088 /
\plot  9.669 19.088  9.605 19.169 /
\plot  9.605 19.169  9.544 19.247 /
\plot  9.544 19.247  9.485 19.325 /
\plot  9.485 19.325  9.426 19.399 /
\plot  9.426 19.399  9.366 19.473 /
\plot  9.366 19.473  9.269 19.594 /
\plot  9.269 19.594  9.174 19.713 /
\plot  9.174 19.713  9.083 19.827 /
\plot  9.083 19.827  8.992 19.937 /
\plot  8.992 19.937  8.903 20.043 /
\plot  8.903 20.043  8.816 20.146 /
\plot  8.816 20.146  8.729 20.248 /
\plot  8.729 20.248  8.644 20.345 /
\plot  8.644 20.345  8.562 20.441 /
\plot  8.562 20.441  8.481 20.534 /
\plot  8.481 20.534  8.401 20.623 /
\plot  8.401 20.623  8.323 20.709 /
\plot  8.323 20.709  8.244 20.792 /
\plot  8.244 20.792  8.168 20.872 /
\plot  8.168 20.872  8.094 20.951 /
\plot  8.094 20.951  8.020 21.025 /
\plot  8.020 21.025  7.948 21.097 /
\plot  7.948 21.097  7.878 21.167 /
\plot  7.878 21.167  7.811 21.232 /
\plot  7.811 21.232  7.745 21.294 /
\plot  7.745 21.294  7.679 21.353 /
\plot  7.679 21.353  7.618 21.410 /
\plot  7.618 21.410  7.557 21.463 /
\plot  7.557 21.463  7.497 21.514 /
\plot  7.497 21.514  7.440 21.560 /
\plot  7.440 21.560  7.385 21.605 /
\plot  7.385 21.605  7.330 21.647 /
\plot  7.330 21.647  7.279 21.685 /
\plot  7.279 21.685  7.228 21.721 /
\plot  7.228 21.721  7.182 21.755 /
\plot  7.182 21.755  7.135 21.787 /
\plot  7.135 21.787  7.089 21.816 /
\plot  7.089 21.816  7.046 21.844 /
\plot  7.046 21.844  7.004 21.867 /
\plot  7.004 21.867  6.964 21.891 /
\plot  6.964 21.891  6.924 21.914 /
\plot  6.924 21.914  6.886 21.933 /
\plot  6.886 21.933  6.847 21.952 /
\plot  6.847 21.952  6.809 21.971 /
\plot  6.809 21.971  6.773 21.986 /
\plot  6.773 21.986  6.714 22.013 /
\plot  6.714 22.013  6.653 22.037 /
\plot  6.653 22.037  6.593 22.060 /
\plot  6.593 22.060  6.534 22.081 /
\plot  6.534 22.081  6.475 22.098 /
\plot  6.475 22.098  6.416 22.115 /
\plot  6.416 22.115  6.356 22.130 /
\plot  6.356 22.130  6.299 22.145 /
\plot  6.299 22.145  6.240 22.155 /
\plot  6.240 22.155  6.183 22.164 /
\plot  6.183 22.164  6.126 22.172 /
\plot  6.126 22.172  6.068 22.176 /
\plot  6.068 22.176  6.016 22.181 /
\plot  6.016 22.181  5.963 22.183 /
\putrule from  5.963 22.183 to  5.912 22.183
\plot  5.912 22.183  5.863 22.181 /
\plot  5.863 22.181  5.817 22.178 /
\plot  5.817 22.178  5.772 22.174 /
\plot  5.772 22.174  5.732 22.168 /
\plot  5.732 22.168  5.692 22.159 /
\plot  5.692 22.159  5.656 22.151 /
\plot  5.656 22.151  5.620 22.142 /
\plot  5.620 22.142  5.588 22.130 /
\plot  5.588 22.130  5.556 22.119 /
\plot  5.556 22.119  5.518 22.102 /
\plot  5.518 22.102  5.480 22.083 /
\plot  5.480 22.083  5.446 22.060 /
\plot  5.446 22.060  5.412 22.035 /
\plot  5.412 22.035  5.378 22.007 /
\plot  5.378 22.007  5.347 21.973 /
\plot  5.347 21.973  5.313 21.935 /
\plot  5.313 21.935  5.279 21.895 /
\plot  5.279 21.895  5.245 21.848 /
\plot  5.245 21.848  5.211 21.800 /
\plot  5.211 21.800  5.179 21.753 /
\plot  5.179 21.753  5.150 21.706 /
\plot  5.150 21.706  5.124 21.666 /
\plot  5.124 21.666  5.105 21.632 /
\plot  5.105 21.632  5.091 21.609 /
\plot  5.091 21.609  5.084 21.596 /
\plot  5.084 21.596  5.080 21.590 /
}%
%
% Fig TEXT object
%
\put{\SetFigFont{6}{7.2}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\tilde{S}_-$}%
} [lB] at  3.810 16.510
%
% Fig TEXT object
%
\put{\SetFigFont{6}{7.2}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\bar{N}_-$}%
} [lB] at  3.810 11.430
%
% Fig TEXT object
%
\put{\SetFigFont{6}{7.2}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\tilde{N}_-$}%
} [lB] at  3.810 21.590
%
% Fig TEXT object
%
\put{\SetFigFont{6}{7.2}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\tilde{S}_+$}%
} [lB] at 15.558 11.430
%
% Fig TEXT object
%
\put{\SetFigFont{6}{7.2}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\tilde{N}_+$}%
} [lB] at 15.558 16.510
%
% Fig TEXT object
%
\put{\SetFigFont{6}{7.2}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\bar{N}_+$}%
} [lB] at 15.558  6.350
%
% Fig TEXT object
%
\put{\SetFigFont{6}{7.2}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\cW^-$}%
} [lB] at 10.478  9.842
%
% Fig TEXT object
%
\put{\SetFigFont{6}{7.2}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\cW^+$}%
} [lB] at  9.842 19.050
%
% Fig TEXT object
%
\put{\SetFigFont{6}{7.2}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\Ga_r$}%
} [lB] at  5.715 12.700
%
% Fig TEXT object
%
\put{\SetFigFont{6}{7.2}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\Ga_l$}%
} [lB] at 14.287 14.605
\linethickness=0pt
\putrectangle corners at  3.778 22.229 and 15.589  5.709
\endpicture}


==> KTZ_zGKN_I_thcor2.tex <==
%Title: /tmp/xfig-fig008064
%%Created by: fig2dev Version 3.2 Patchlevel 5
%%CreationDate: Wed Feb 18 13:00:43 1970
%%User: shadi@attar (Tahvildar-Zadeh A. Shadi)
\font\thinlinefont=cmr5
%
\begingroup\makeatletter\ifx\SetFigFont\undefined%
\gdef\SetFigFont#1#2#3#4#5{%
  \reset@font\fontsize{#1}{#2pt}%
  \fontfamily{#3}\fontseries{#4}\fontshape{#5}%
  \selectfont}%
\fi\endgroup%
\mbox{\beginpicture
\setcoordinatesystem units <0.50000cm,0.50000cm>
\unitlength=0.50000cm
\linethickness=1pt
\setplotsymbol ({\makebox(0,0)[l]{\tencirc\symbol{'160}}})
\setshadesymbol ({\thinlinefont .})
\setlinear
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\putrule from  5.080 16.510 to 15.240 16.510
}%
%
% Fig POLYLINE object
%
\linethickness=1pt
\setplotsymbol ({\makebox(0,0)[l]{\tencirc\symbol{'160}}})
{\color[rgb]{0,0,0}\putrule from  5.080 21.590 to 15.240 21.590
}%
%
% Fig POLYLINE object
%
\linethickness=1pt
\setplotsymbol ({\makebox(0,0)[l]{\tencirc\symbol{'160}}})
{\color[rgb]{0,0,0}\putrule from 15.240 21.590 to 15.240  6.315
\putrule from 15.240  6.350 to  5.045  6.350
\putrule from  5.080  6.350 to  5.080 21.590
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\putrule from  5.080 11.430 to 15.240 11.430
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  7.938 14.287  9.684 13.970 /
%
% arrow head
%
\plot  9.422 13.953  9.684 13.970  9.445 14.078 /
%
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot 11.906 13.018 13.335 12.859 /
%
% arrow head
%
\plot 13.076 12.824 13.335 12.859 13.090 12.950 /
%
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  7.620 16.828  9.366 16.192 /
%
% arrow head
%
\plot  9.106 16.220  9.366 16.192  9.149 16.339 /
%
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot 12.224 16.828 13.652 16.192 /
%
% arrow head
%
\plot 13.395 16.238 13.652 16.192 13.446 16.354 /
%
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\putrule from 15.240 12.700 to 15.240 13.970
%
% arrow head
%
\plot 15.304 13.716 15.240 13.970 15.176 13.716 /
%
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  5.715 16.510  7.620 14.605 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  6.985 16.510  9.684 13.811 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  8.255 16.510 11.430 13.335 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  9.525 16.510 13.494 12.541 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot 10.795 16.510 15.240 12.065 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot 12.065 16.510 15.240 13.335 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot 13.335 16.510 15.240 14.605 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot 14.605 16.510 15.240 15.875 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  5.080 16.510  5.082 16.506 /
\plot  5.082 16.506  5.086 16.493 /
\plot  5.086 16.493  5.093 16.474 /
\plot  5.093 16.474  5.103 16.442 /
\plot  5.103 16.442  5.118 16.398 /
\plot  5.118 16.398  5.137 16.343 /
\plot  5.137 16.343  5.160 16.277 /
\plot  5.160 16.277  5.186 16.201 /
\plot  5.186 16.201  5.215 16.116 /
\plot  5.215 16.116  5.245 16.025 /
\plot  5.245 16.025  5.277 15.932 /
\plot  5.277 15.932  5.309 15.839 /
\plot  5.309 15.839  5.338 15.744 /
\plot  5.338 15.744  5.368 15.653 /
\plot  5.368 15.653  5.395 15.564 /
\plot  5.395 15.564  5.423 15.477 /
\plot  5.423 15.477  5.448 15.397 /
\plot  5.448 15.397  5.472 15.318 /
\plot  5.472 15.318  5.493 15.244 /
\plot  5.493 15.244  5.512 15.174 /
\plot  5.512 15.174  5.529 15.107 /
\plot  5.529 15.107  5.546 15.041 /
\plot  5.546 15.041  5.560 14.978 /
\plot  5.560 14.978  5.573 14.916 /
\plot  5.573 14.916  5.586 14.857 /
\plot  5.586 14.857  5.599 14.798 /
\plot  5.599 14.798  5.609 14.736 /
\plot  5.609 14.736  5.620 14.677 /
\plot  5.620 14.677  5.628 14.618 /
\plot  5.628 14.618  5.637 14.556 /
\plot  5.637 14.556  5.645 14.493 /
\plot  5.645 14.493  5.654 14.431 /
\plot  5.654 14.431  5.660 14.366 /
\plot  5.660 14.366  5.666 14.300 /
\plot  5.666 14.300  5.671 14.235 /
\plot  5.671 14.235  5.675 14.167 /
\plot  5.675 14.167  5.679 14.097 /
\plot  5.679 14.097  5.681 14.029 /
\plot  5.681 14.029  5.683 13.959 /
\plot  5.683 13.959  5.685 13.890 /
\putrule from  5.685 13.890 to  5.685 13.818
\putrule from  5.685 13.818 to  5.685 13.748
\plot  5.685 13.748  5.683 13.680 /
\plot  5.683 13.680  5.681 13.610 /
\plot  5.681 13.610  5.679 13.542 /
\plot  5.679 13.542  5.675 13.477 /
\plot  5.675 13.477  5.671 13.411 /
\plot  5.671 13.411  5.666 13.346 /
\plot  5.666 13.346  5.660 13.284 /
\plot  5.660 13.284  5.654 13.223 /
\plot  5.654 13.223  5.645 13.164 /
\plot  5.645 13.164  5.637 13.106 /
\plot  5.637 13.106  5.628 13.049 /
\plot  5.628 13.049  5.620 12.992 /
\plot  5.620 12.992  5.609 12.937 /
\plot  5.609 12.937  5.599 12.880 /
\plot  5.599 12.880  5.586 12.821 /
\plot  5.586 12.821  5.571 12.764 /
\plot  5.571 12.764  5.556 12.704 /
\plot  5.556 12.704  5.539 12.645 /
\plot  5.539 12.645  5.520 12.581 /
\plot  5.520 12.581  5.501 12.518 /
\plot  5.501 12.518  5.480 12.450 /
\plot  5.480 12.450  5.455 12.380 /
\plot  5.455 12.380  5.429 12.306 /
\plot  5.429 12.306  5.400 12.230 /
\plot  5.400 12.230  5.370 12.150 /
\plot  5.370 12.150  5.338 12.067 /
\plot  5.338 12.067  5.304 11.982 /
\plot  5.304 11.982  5.273 11.898 /
\plot  5.273 11.898  5.239 11.813 /
\plot  5.239 11.813  5.207 11.735 /
\plot  5.207 11.735  5.175 11.661 /
\plot  5.175 11.661  5.150 11.597 /
\plot  5.150 11.597  5.127 11.542 /
\plot  5.127 11.542  5.110 11.498 /
\plot  5.110 11.498  5.095 11.468 /
\plot  5.095 11.468  5.086 11.447 /
\plot  5.086 11.447  5.082 11.434 /
\plot  5.082 11.434  5.080 11.430 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot 15.240 16.510 15.238 16.506 /
\plot 15.238 16.506 15.234 16.493 /
\plot 15.234 16.493 15.227 16.474 /
\plot 15.227 16.474 15.217 16.442 /
\plot 15.217 16.442 15.202 16.398 /
\plot 15.202 16.398 15.183 16.343 /
\plot 15.183 16.343 15.160 16.275 /
\plot 15.160 16.275 15.134 16.199 /
\plot 15.134 16.199 15.105 16.114 /
\plot 15.105 16.114 15.075 16.023 /
\plot 15.075 16.023 15.043 15.930 /
\plot 15.043 15.930 15.011 15.835 /
\plot 15.011 15.835 14.982 15.740 /
\plot 14.982 15.740 14.952 15.646 /
\plot 14.952 15.646 14.925 15.558 /
\plot 14.925 15.558 14.897 15.471 /
\plot 14.897 15.471 14.872 15.388 /
\plot 14.872 15.388 14.848 15.308 /
\plot 14.848 15.308 14.827 15.234 /
\plot 14.827 15.234 14.808 15.162 /
\plot 14.808 15.162 14.791 15.092 /
\plot 14.791 15.092 14.774 15.026 /
\plot 14.774 15.026 14.760 14.961 /
\plot 14.760 14.961 14.747 14.897 /
\plot 14.747 14.897 14.734 14.836 /
\plot 14.734 14.836 14.721 14.772 /
\plot 14.721 14.772 14.711 14.711 /
\plot 14.711 14.711 14.700 14.647 /
\plot 14.700 14.647 14.692 14.586 /
\plot 14.692 14.586 14.683 14.520 /
\plot 14.683 14.520 14.675 14.455 /
\plot 14.675 14.455 14.666 14.389 /
\plot 14.666 14.389 14.660 14.321 /
\plot 14.660 14.321 14.654 14.252 /
\plot 14.654 14.252 14.649 14.182 /
\plot 14.649 14.182 14.645 14.110 /
\plot 14.645 14.110 14.641 14.038 /
\plot 14.641 14.038 14.639 13.964 /
\plot 14.639 13.964 14.637 13.892 /
\plot 14.637 13.892 14.635 13.818 /
\putrule from 14.635 13.818 to 14.635 13.744
\putrule from 14.635 13.744 to 14.635 13.669
\plot 14.635 13.669 14.637 13.595 /
\plot 14.637 13.595 14.639 13.523 /
\plot 14.639 13.523 14.641 13.454 /
\plot 14.641 13.454 14.645 13.384 /
\plot 14.645 13.384 14.649 13.316 /
\plot 14.649 13.316 14.654 13.248 /
\plot 14.654 13.248 14.660 13.185 /
\plot 14.660 13.185 14.666 13.121 /
\plot 14.666 13.121 14.675 13.060 /
\plot 14.675 13.060 14.683 13.001 /
\plot 14.683 13.001 14.692 12.943 /
\plot 14.692 12.943 14.700 12.888 /
\plot 14.700 12.888 14.711 12.831 /
\plot 14.711 12.831 14.721 12.774 /
\plot 14.721 12.774 14.734 12.717 /
\plot 14.734 12.717 14.749 12.660 /
\plot 14.749 12.660 14.764 12.603 /
\plot 14.764 12.603 14.781 12.543 /
\plot 14.781 12.543 14.800 12.486 /
\plot 14.800 12.486 14.819 12.425 /
\plot 14.819 12.425 14.840 12.361 /
\plot 14.840 12.361 14.865 12.296 /
\plot 14.865 12.296 14.891 12.228 /
\plot 14.891 12.228 14.920 12.156 /
\plot 14.920 12.156 14.950 12.082 /
\plot 14.950 12.082 14.982 12.006 /
\plot 14.982 12.006 15.016 11.930 /
\plot 15.016 11.930 15.047 11.851 /
\plot 15.047 11.851 15.081 11.777 /
\plot 15.081 11.777 15.113 11.705 /
\plot 15.113 11.705 15.145 11.637 /
\plot 15.145 11.637 15.170 11.580 /
\plot 15.170 11.580 15.193 11.532 /
\plot 15.193 11.532 15.210 11.491 /
\plot 15.210 11.491 15.225 11.464 /
\plot 15.225 11.464 15.234 11.445 /
\plot 15.234 11.445 15.238 11.434 /
\plot 15.238 11.434 15.240 11.430 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  5.080 16.510  5.082 16.508 /
\plot  5.082 16.508  5.086 16.504 /
\plot  5.086 16.504  5.095 16.493 /
\plot  5.095 16.493  5.108 16.478 /
\plot  5.108 16.478  5.127 16.457 /
\plot  5.127 16.457  5.150 16.430 /
\plot  5.150 16.430  5.182 16.396 /
\plot  5.182 16.396  5.220 16.353 /
\plot  5.220 16.353  5.264 16.305 /
\plot  5.264 16.305  5.315 16.248 /
\plot  5.315 16.248  5.372 16.188 /
\plot  5.372 16.188  5.433 16.121 /
\plot  5.433 16.121  5.499 16.053 /
\plot  5.499 16.053  5.571 15.979 /
\plot  5.571 15.979  5.643 15.905 /
\plot  5.643 15.905  5.719 15.831 /
\plot  5.719 15.831  5.798 15.754 /
\plot  5.798 15.754  5.876 15.680 /
\plot  5.876 15.680  5.956 15.606 /
\plot  5.956 15.606  6.035 15.534 /
\plot  6.035 15.534  6.115 15.464 /
\plot  6.115 15.464  6.195 15.397 /
\plot  6.195 15.397  6.274 15.331 /
\plot  6.274 15.331  6.354 15.268 /
\plot  6.354 15.268  6.435 15.208 /
\plot  6.435 15.208  6.515 15.149 /
\plot  6.515 15.149  6.596 15.094 /
\plot  6.596 15.094  6.678 15.039 /
\plot  6.678 15.039  6.763 14.986 /
\plot  6.763 14.986  6.847 14.935 /
\plot  6.847 14.935  6.934 14.887 /
\plot  6.934 14.887  7.023 14.838 /
\plot  7.023 14.838  7.114 14.791 /
\plot  7.114 14.791  7.209 14.743 /
\plot  7.209 14.743  7.307 14.696 /
\plot  7.307 14.696  7.408 14.652 /
\plot  7.408 14.652  7.514 14.605 /
\plot  7.514 14.605  7.597 14.569 /
\plot  7.597 14.569  7.681 14.535 /
\plot  7.681 14.535  7.768 14.499 /
\plot  7.768 14.499  7.859 14.465 /
\plot  7.859 14.465  7.950 14.429 /
\plot  7.950 14.429  8.045 14.393 /
\plot  8.045 14.393  8.141 14.357 /
\plot  8.141 14.357  8.240 14.321 /
\plot  8.240 14.321  8.342 14.285 /
\plot  8.342 14.285  8.448 14.247 /
\plot  8.448 14.247  8.553 14.211 /
\plot  8.553 14.211  8.664 14.173 /
\plot  8.664 14.173  8.774 14.135 /
\plot  8.774 14.135  8.888 14.097 /
\plot  8.888 14.097  9.002 14.059 /
\plot  9.002 14.059  9.121 14.021 /
\plot  9.121 14.021  9.239 13.981 /
\plot  9.239 13.981  9.360 13.942 /
\plot  9.360 13.942  9.483 13.904 /
\plot  9.483 13.904  9.605 13.864 /
\plot  9.605 13.864  9.730 13.824 /
\plot  9.730 13.824  9.857 13.786 /
\plot  9.857 13.786  9.982 13.746 /
\plot  9.982 13.746 10.109 13.705 /
\plot 10.109 13.705 10.236 13.667 /
\plot 10.236 13.667 10.363 13.627 /
\plot 10.363 13.627 10.488 13.589 /
\plot 10.488 13.589 10.615 13.551 /
\plot 10.615 13.551 10.740 13.513 /
\plot 10.740 13.513 10.865 13.473 /
\plot 10.865 13.473 10.988 13.437 /
\plot 10.988 13.437 11.108 13.399 /
\plot 11.108 13.399 11.229 13.360 /
\plot 11.229 13.360 11.347 13.324 /
\plot 11.347 13.324 11.466 13.288 /
\plot 11.466 13.288 11.580 13.252 /
\plot 11.580 13.252 11.692 13.219 /
\plot 11.692 13.219 11.803 13.183 /
\plot 11.803 13.183 11.910 13.149 /
\plot 11.910 13.149 12.016 13.115 /
\plot 12.016 13.115 12.120 13.083 /
\plot 12.120 13.083 12.222 13.049 /
\plot 12.222 13.049 12.319 13.018 /
\plot 12.319 13.018 12.416 12.986 /
\plot 12.416 12.986 12.509 12.956 /
\plot 12.509 12.956 12.601 12.924 /
\plot 12.601 12.924 12.687 12.895 /
\plot 12.687 12.895 12.774 12.865 /
\plot 12.774 12.865 12.857 12.835 /
\plot 12.857 12.835 12.937 12.806 /
\putrule from 12.937 12.806 to 12.939 12.806
\plot 12.939 12.806 13.053 12.764 /
\plot 13.053 12.764 13.164 12.721 /
\plot 13.164 12.721 13.269 12.679 /
\plot 13.269 12.679 13.371 12.636 /
\plot 13.371 12.636 13.470 12.594 /
\plot 13.470 12.594 13.566 12.552 /
\plot 13.566 12.552 13.657 12.509 /
\plot 13.657 12.509 13.746 12.465 /
\plot 13.746 12.465 13.835 12.421 /
\plot 13.835 12.421 13.921 12.374 /
\plot 13.921 12.374 14.006 12.325 /
\plot 14.006 12.325 14.091 12.275 /
\plot 14.091 12.275 14.175 12.224 /
\plot 14.175 12.224 14.260 12.171 /
\plot 14.260 12.171 14.343 12.116 /
\plot 14.343 12.116 14.425 12.059 /
\plot 14.425 12.059 14.510 12.002 /
\plot 14.510 12.002 14.590 11.944 /
\plot 14.590 11.944 14.671 11.885 /
\plot 14.671 11.885 14.747 11.826 /
\plot 14.747 11.826 14.823 11.769 /
\plot 14.823 11.769 14.893 11.716 /
\plot 14.893 11.716 14.958 11.663 /
\plot 14.958 11.663 15.018 11.616 /
\plot 15.018 11.616 15.071 11.572 /
\plot 15.071 11.572 15.115 11.536 /
\plot 15.115 11.536 15.153 11.504 /
\plot 15.153 11.504 15.183 11.479 /
\plot 15.183 11.479 15.206 11.460 /
\plot 15.206 11.460 15.223 11.445 /
\plot 15.223 11.445 15.232 11.436 /
\plot 15.232 11.436 15.238 11.432 /
\plot 15.238 11.432 15.240 11.430 /
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot  5.080 16.510  5.084 16.506 /
\plot  5.084 16.506  5.091 16.499 /
\plot  5.091 16.499  5.105 16.487 /
\plot  5.105 16.487  5.127 16.466 /
\plot  5.127 16.466  5.156 16.438 /
\plot  5.156 16.438  5.194 16.402 /
\plot  5.194 16.402  5.241 16.360 /
\plot  5.241 16.360  5.292 16.313 /
\plot  5.292 16.313  5.347 16.260 /
\plot  5.347 16.260  5.406 16.207 /
\plot  5.406 16.207  5.465 16.154 /
\plot  5.465 16.154  5.527 16.099 /
\plot  5.527 16.099  5.588 16.046 /
\plot  5.588 16.046  5.645 15.996 /
\plot  5.645 15.996  5.702 15.949 /
\plot  5.702 15.949  5.759 15.903 /
\plot  5.759 15.903  5.812 15.860 /
\plot  5.812 15.860  5.863 15.820 /
\plot  5.863 15.820  5.914 15.782 /
\plot  5.914 15.782  5.965 15.746 /
\plot  5.965 15.746  6.013 15.712 /
\plot  6.013 15.712  6.064 15.678 /
\plot  6.064 15.678  6.115 15.646 /
\plot  6.115 15.646  6.166 15.615 /
\plot  6.166 15.615  6.219 15.583 /
\plot  6.219 15.583  6.259 15.560 /
\plot  6.259 15.560  6.301 15.536 /
\plot  6.301 15.536  6.344 15.513 /
\plot  6.344 15.513  6.390 15.490 /
\plot  6.390 15.490  6.437 15.466 /
\plot  6.437 15.466  6.485 15.443 /
\plot  6.485 15.443  6.536 15.418 /
\plot  6.536 15.418  6.591 15.395 /
\plot  6.591 15.395  6.646 15.369 /
\plot  6.646 15.369  6.703 15.344 /
\plot  6.703 15.344  6.765 15.318 /
\plot  6.765 15.318  6.828 15.295 /
\plot  6.828 15.295  6.894 15.270 /
\plot  6.894 15.270  6.964 15.244 /
\plot  6.964 15.244  7.036 15.219 /
\plot  7.036 15.219  7.110 15.193 /
\plot  7.110 15.193  7.186 15.168 /
\plot  7.186 15.168  7.264 15.143 /
\plot  7.264 15.143  7.345 15.117 /
\plot  7.345 15.117  7.429 15.094 /
\plot  7.429 15.094  7.514 15.069 /
\plot  7.514 15.069  7.601 15.045 /
\plot  7.601 15.045  7.690 15.022 /
\plot  7.690 15.022  7.781 14.999 /
\plot  7.781 14.999  7.874 14.975 /
\plot  7.874 14.975  7.967 14.954 /
\plot  7.967 14.954  8.062 14.931 /
\plot  8.062 14.931  8.160 14.910 /
\plot  8.160 14.910  8.259 14.889 /
\plot  8.259 14.889  8.361 14.870 /
\plot  8.361 14.870  8.462 14.848 /
\plot  8.462 14.848  8.568 14.829 /
\plot  8.568 14.829  8.674 14.810 /
\plot  8.674 14.810  8.784 14.789 /
\plot  8.784 14.789  8.867 14.776 /
\plot  8.867 14.776  8.951 14.762 /
\plot  8.951 14.762  9.038 14.747 /
\plot  9.038 14.747  9.129 14.734 /
\plot  9.129 14.734  9.220 14.719 /
\plot  9.220 14.719  9.313 14.704 /
\plot  9.313 14.704  9.409 14.692 /
\plot  9.409 14.692  9.506 14.677 /
\plot  9.506 14.677  9.605 14.662 /
\plot  9.605 14.662  9.707 14.647 /
\plot  9.707 14.647  9.811 14.635 /
\plot  9.811 14.635  9.914 14.620 /
\plot  9.914 14.620 10.022 14.605 /
\plot 10.022 14.605 10.132 14.590 /
\plot 10.132 14.590 10.243 14.577 /
\plot 10.243 14.577 10.355 14.563 /
\plot 10.355 14.563 10.467 14.548 /
\plot 10.467 14.548 10.581 14.533 /
\plot 10.581 14.533 10.696 14.520 /
\plot 10.696 14.520 10.812 14.506 /
\plot 10.812 14.506 10.926 14.493 /
\plot 10.926 14.493 11.043 14.478 /
\plot 11.043 14.478 11.159 14.465 /
\plot 11.159 14.465 11.273 14.450 /
\plot 11.273 14.450 11.390 14.438 /
\plot 11.390 14.438 11.504 14.425 /
\plot 11.504 14.425 11.616 14.412 /
\plot 11.616 14.412 11.728 14.400 /
\plot 11.728 14.400 11.839 14.389 /
\plot 11.839 14.389 11.946 14.376 /
\plot 11.946 14.376 12.052 14.366 /
\plot 12.052 14.366 12.158 14.353 /
\plot 12.158 14.353 12.260 14.343 /
\plot 12.260 14.343 12.361 14.332 /
\plot 12.361 14.332 12.459 14.323 /
\plot 12.459 14.323 12.554 14.313 /
\plot 12.554 14.313 12.647 14.304 /
\plot 12.647 14.304 12.736 14.294 /
\plot 12.736 14.294 12.823 14.285 /
\plot 12.823 14.285 12.907 14.277 /
\plot 12.907 14.277 12.990 14.271 /
\plot 12.990 14.271 13.070 14.262 /
\plot 13.070 14.262 13.147 14.256 /
\plot 13.147 14.256 13.221 14.247 /
\plot 13.221 14.247 13.293 14.241 /
\plot 13.293 14.241 13.363 14.235 /
\plot 13.363 14.235 13.464 14.226 /
\plot 13.464 14.226 13.559 14.216 /
\plot 13.559 14.216 13.652 14.209 /
\plot 13.652 14.209 13.739 14.201 /
\plot 13.739 14.201 13.824 14.194 /
\plot 13.824 14.194 13.904 14.190 /
\plot 13.904 14.190 13.981 14.186 /
\plot 13.981 14.186 14.055 14.182 /
\plot 14.055 14.182 14.125 14.180 /
\putrule from 14.125 14.180 to 14.190 14.180
\putrule from 14.190 14.180 to 14.254 14.180
\plot 14.254 14.180 14.313 14.182 /
\plot 14.313 14.182 14.368 14.186 /
\plot 14.368 14.186 14.421 14.192 /
\plot 14.421 14.192 14.470 14.199 /
\plot 14.470 14.199 14.514 14.207 /
\plot 14.514 14.207 14.556 14.218 /
\plot 14.556 14.218 14.594 14.230 /
\plot 14.594 14.230 14.630 14.245 /
\plot 14.630 14.245 14.662 14.262 /
\plot 14.662 14.262 14.692 14.279 /
\plot 14.692 14.279 14.719 14.300 /
\plot 14.719 14.300 14.745 14.321 /
\plot 14.745 14.321 14.766 14.345 /
\plot 14.766 14.345 14.787 14.370 /
\plot 14.787 14.370 14.806 14.398 /
\plot 14.806 14.398 14.823 14.427 /
\plot 14.823 14.427 14.840 14.457 /
\plot 14.840 14.457 14.855 14.491 /
\plot 14.855 14.491 14.870 14.525 /
\plot 14.870 14.525 14.884 14.563 /
\plot 14.884 14.563 14.897 14.603 /
\plot 14.897 14.603 14.912 14.647 /
\plot 14.912 14.647 14.927 14.694 /
\plot 14.927 14.694 14.939 14.745 /
\plot 14.939 14.745 14.954 14.800 /
\plot 14.954 14.800 14.967 14.861 /
\plot 14.967 14.861 14.982 14.925 /
\plot 14.982 14.925 14.997 14.997 /
\plot 14.997 14.997 15.011 15.073 /
\plot 15.011 15.073 15.026 15.155 /
\plot 15.026 15.155 15.043 15.242 /
\plot 15.043 15.242 15.058 15.337 /
\plot 15.058 15.337 15.075 15.437 /
\plot 15.075 15.437 15.092 15.541 /
\plot 15.092 15.541 15.109 15.649 /
\plot 15.109 15.649 15.128 15.756 /
\plot 15.128 15.756 15.145 15.867 /
\plot 15.145 15.867 15.160 15.972 /
\plot 15.160 15.972 15.176 16.076 /
\plot 15.176 16.076 15.189 16.169 /
\plot 15.189 16.169 15.202 16.256 /
\plot 15.202 16.256 15.215 16.328 /
\plot 15.215 16.328 15.223 16.389 /
\plot 15.223 16.389 15.229 16.436 /
\plot 15.229 16.436 15.234 16.470 /
\plot 15.234 16.470 15.238 16.493 /
\plot 15.238 16.493 15.240 16.504 /
\putrule from 15.240 16.504 to 15.240 16.510
}%
%
% Fig POLYLINE object
%
\linethickness= 0.500pt
\setplotsymbol ({\thinlinefont .})
{\color[rgb]{0,0,0}\plot 15.240 11.430 15.238 11.432 /
\plot 15.238 11.432 15.232 11.434 /
\plot 15.232 11.434 15.221 11.441 /
\plot 15.221 11.441 15.206 11.451 /
\plot 15.206 11.451 15.183 11.466 /
\plot 15.183 11.466 15.153 11.483 /
\plot 15.153 11.483 15.115 11.506 /
\plot 15.115 11.506 15.069 11.532 /
\plot 15.069 11.532 15.018 11.561 /
\plot 15.018 11.561 14.961 11.593 /
\plot 14.961 11.593 14.897 11.627 /
\plot 14.897 11.627 14.829 11.663 /
\plot 14.829 11.663 14.757 11.699 /
\plot 14.757 11.699 14.683 11.735 /
\plot 14.683 11.735 14.609 11.771 /
\plot 14.609 11.771 14.531 11.805 /
\plot 14.531 11.805 14.450 11.841 /
\plot 14.450 11.841 14.368 11.874 /
\plot 14.368 11.874 14.285 11.906 /
\plot 14.285 11.906 14.199 11.938 /
\plot 14.199 11.938 14.110 11.970 /
\plot 14.110 11.970 14.019 12.002 /
\plot 14.019 12.002 13.921 12.033 /
\plot 13.921 12.033 13.822 12.063 /
\plot 13.822 12.063 13.716 12.095 /
\plot 13.716 12.095 13.604 12.126 /
\plot 13.604 12.126 13.485 12.158 /
\plot 13.485 12.158 13.360 12.190 /
\plot 13.360 12.190 13.229 12.224 /
\plot 13.229 12.224 13.149 12.243 /
\plot 13.149 12.243 13.068 12.264 /
\plot 13.068 12.264 12.984 12.283 /
\plot 12.984 12.283 12.897 12.304 /
\plot 12.897 12.304 12.806 12.325 /
\plot 12.806 12.325 12.713 12.349 /
\plot 12.713 12.349 12.617 12.370 /
\plot 12.617 12.370 12.520 12.391 /
\plot 12.520 12.391 12.421 12.414 /
\plot 12.421 12.414 12.317 12.438 /
\plot 12.317 12.438 12.211 12.461 /
\plot 12.211 12.461 12.103 12.486 /
\plot 12.103 12.486 11.993 12.509 /
\plot 11.993 12.509 11.881 12.535 /
\plot 11.881 12.535 11.764 12.558 /
\plot 11.764 12.558 11.648 12.584 /
\plot 11.648 12.584 11.527 12.609 /
\plot 11.527 12.609 11.407 12.634 /
\plot 11.407 12.634 11.284 12.662 /
\plot 11.284 12.662 11.161 12.687 /
\plot 11.161 12.687 11.034 12.713 /
\plot 11.034 12.713 10.907 12.740 /
\plot 10.907 12.740 10.780 12.766 /
\plot 10.780 12.766 10.653 12.791 /
\plot 10.653 12.791 10.524 12.819 /
\plot 10.524 12.819 10.395 12.844 /
\plot 10.395 12.844 10.266 12.869 /
\plot 10.266 12.869 10.137 12.897 /
\plot 10.137 12.897 10.008 12.922 /
\plot 10.008 12.922  9.881 12.948 /
\plot  9.881 12.948  9.754 12.973 /
\plot  9.754 12.973  9.627 12.996 /
\plot  9.627 12.996  9.504 13.022 /
\plot  9.504 13.022  9.379 13.045 /
\plot  9.379 13.045  9.258 13.068 /
\plot  9.258 13.068  9.138 13.092 /
\plot  9.138 13.092  9.021 13.115 /
\plot  9.021 13.115  8.905 13.136 /
\plot  8.905 13.136  8.791 13.159 /
\plot  8.791 13.159  8.680 13.180 /
\plot  8.680 13.180  8.570 13.200 /
\plot  8.570 13.200  8.465 13.221 /
\plot  8.465 13.221  8.361 13.240 /
\plot  8.361 13.240  8.259 13.259 /
\plot  8.259 13.259  8.160 13.276 /
\plot  8.160 13.276  8.064 13.295 /
\plot  8.064 13.295  7.969 13.312 /
\plot  7.969 13.312  7.878 13.329 /
\plot  7.878 13.329  7.791 13.343 /
\plot  7.791 13.343  7.705 13.358 /
\plot  7.705 13.358  7.622 13.373 /
\plot  7.622 13.373  7.542 13.388 /
\plot  7.542 13.388  7.415 13.409 /
\plot  7.415 13.409  7.294 13.430 /
\plot  7.294 13.430  7.178 13.449 /
\plot  7.178 13.449  7.065 13.468 /
\plot  7.065 13.468  6.960 13.485 /
\plot  6.960 13.485  6.856 13.500 /
\plot  6.856 13.500  6.759 13.515 /
\plot  6.759 13.515  6.663 13.528 /
\plot  6.663 13.528  6.574 13.538 /
\plot  6.574 13.538  6.488 13.547 /
\plot  6.488 13.547  6.405 13.555 /
\plot  6.405 13.555  6.327 13.559 /
\plot  6.327 13.559  6.253 13.564 /
\plot  6.253 13.564  6.183 13.566 /
\putrule from  6.183 13.566 to  6.115 13.566
\plot  6.115 13.566  6.054 13.564 /
\plot  6.054 13.564  5.994 13.561 /
\plot  5.994 13.561  5.941 13.555 /
\plot  5.941 13.555  5.891 13.547 /
\plot  5.891 13.547  5.844 13.538 /
\plot  5.844 13.538  5.802 13.526 /
\plot  5.802 13.526  5.762 13.513 /
\plot  5.762 13.513  5.726 13.498 /
\plot  5.726 13.498  5.692 13.481 /
\plot  5.692 13.481  5.660 13.462 /
\plot  5.660 13.462  5.632 13.441 /
\plot  5.632 13.441  5.607 13.420 /
\plot  5.607 13.420  5.584 13.394 /
\plot  5.584 13.394  5.563 13.369 /
\plot  5.563 13.369  5.541 13.341 /
\plot  5.541 13.341  5.522 13.314 /
\plot  5.522 13.314  5.503 13.282 /
\plot  5.503 13.282  5.482 13.244 /
\plot  5.482 13.244  5.463 13.204 /
\plot  5.463 13.204  5.444 13.159 /
\plot  5.444 13.159  5.425 13.113 /
\plot  5.425 13.113  5.406 13.060 /
\plot  5.406 13.060  5.389 13.003 /
\plot  5.389 13.003  5.370 12.939 /
\plot  5.370 12.939  5.353 12.871 /
\plot  5.353 12.871  5.334 12.797 /
\plot  5.334 12.797  5.315 12.717 /
\plot  5.315 12.717  5.296 12.630 /
\plot  5.296 12.630  5.277 12.537 /
\plot  5.277 12.537  5.256 12.438 /
\plot  5.256 12.438  5.237 12.334 /
\plot  5.237 12.334  5.215 12.228 /
\plot  5.215 12.228  5.196 12.118 /
\plot  5.196 12.118  5.177 12.010 /
\plot  5.177 12.010  5.158 11.904 /
\plot  5.158 11.904  5.141 11.803 /
\plot  5.141 11.803  5.127 11.712 /
\plot  5.127 11.712  5.112 11.631 /
\plot  5.112 11.631  5.101 11.565 /
\plot  5.101 11.565  5.093 11.513 /
\plot  5.093 11.513  5.086 11.474 /
\plot  5.086 11.474  5.082 11.449 /
\plot  5.082 11.449  5.080 11.436 /
\putrule from  5.080 11.436 to  5.080 11.430
}%
%
% Fig TEXT object
%
\put{\SetFigFont{6}{7.2}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\tilde{S}_-$}%
} [lB] at  3.810 16.510
%
% Fig TEXT object
%
\put{\SetFigFont{6}{7.2}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\bar{N}_-$}%
} [lB] at  3.810 11.430
%
% Fig TEXT object
%
\put{\SetFigFont{6}{7.2}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\tilde{N}_-$}%
} [lB] at  3.810 21.590
%
% Fig TEXT object
%
\put{\SetFigFont{6}{7.2}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\tilde{S}_+$}%
} [lB] at 15.558 11.430
%
% Fig TEXT object
%
\put{\SetFigFont{6}{7.2}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\tilde{N}_+$}%
} [lB] at 15.558 16.510
%
% Fig TEXT object
%
\put{\SetFigFont{6}{7.2}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\bar{N}_+$}%
} [lB] at 15.558  6.350
%
% Fig TEXT object
%
\put{\SetFigFont{6}{7.2}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\Ga_r$}%
} [lB] at  5.715 12.700
%
% Fig TEXT object
%
\put{\SetFigFont{6}{7.2}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\Ga_l$}%
} [lB] at 14.287 14.605
%
% Fig TEXT object
%
\put{\SetFigFont{6}{7.2}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\cS^\Theta(E,\la)$}%
} [lB] at  9.525 13.494
%
% Fig TEXT object
%
\put{\SetFigFont{6}{7.2}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\cR$}%
} [lB] at 11.748 15.558
%
% Fig TEXT object
%
\put{\SetFigFont{6}{7.2}{\rmdefault}{\mddefault}{\updefault}{\color[rgb]{0,0,0}$\cW^-(E',\la)$}%
} [lB] at  7.620 15.081
\linethickness=0pt
\putrectangle corners at  3.778 21.901 and 15.589  6.215
\endpicture}

